A primer on the use of probability generating functions in infectious disease modeling

We explore the application of probability generating functions (PGFs) to invasive processes, focusing on infectious disease introduced into large populations. Our goal is to acquaint the reader with applications of PGFs, moreso than to derive new results. PGFs help predict a number of properties about early outbreak behavior while the population is still effectively infinite, including the probability of an epidemic, the size distribution after some number of generations, and the cumulative size distribution of non-epidemic outbreaks. We show how PGFs can be used in both discrete-time and continuous-time settings, and discuss how to use these results to infer disease parameters from observed outbreaks. In the large population limit for susceptible-infected-recovered (SIR) epidemics PGFs lead to survival-function based models that are equivalent the the usual mass-action SIR models but with fewer ODEs. We use these to explore properties such as the final size of epidemics or even the dynamics once stochastic effects are negligible. We target this tutorial to biologists and public health researchers who want to learn how to apply PGFs to invasive diseases, but it could also be used in an introductory mathematics course on PGFs. We include many exercises to help demonstrate concepts and to give practice applying the results. We summarize our main results in a few tables. Additionally we provide a small python package which performs many of the relevant calculations.

==> PythontexFile.tex <==
\makeatletter
\def\PYGdefault@reset{\let\PYGdefault@it=\relax \let\PYGdefault@bf=\relax%
    \let\PYGdefault@ul=\relax \let\PYGdefault@tc=\relax%
    \let\PYGdefault@bc=\relax \let\PYGdefault@ff=\relax}
\def\PYGdefault@tok#1{\csname PYGdefault@tok@#1\endcsname}
\def\PYGdefault@toks#1+{\ifx\relax#1\empty\else%
    \PYGdefault@tok{#1}\expandafter\PYGdefault@toks\fi}
\def\PYGdefault@do#1{\PYGdefault@bc{\PYGdefault@tc{\PYGdefault@ul{%
    \PYGdefault@it{\PYGdefault@bf{\PYGdefault@ff{#1}}}}}}}
\def\PYGdefault#1#2{\PYGdefault@reset\PYGdefault@toks#1+\relax+\PYGdefault@do{#2}}

\expandafter\def\csname PYGdefault@tok@gd\endcsname{\def\PYGdefault@tc##1{\textcolor[rgb]{0.63,0.00,0.00}{##1}}}
\expandafter\def\csname PYGdefault@tok@gu\endcsname{\let\PYGdefault@bf=\textbf\def\PYGdefault@tc##1{\textcolor[rgb]{0.50,0.00,0.50}{##1}}}
\expandafter\def\csname PYGdefault@tok@gt\endcsname{\def\PYGdefault@tc##1{\textcolor[rgb]{0.00,0.27,0.87}{##1}}}
\expandafter\def\csname PYGdefault@tok@gs\endcsname{\let\PYGdefault@bf=\textbf}
\expandafter\def\csname PYGdefault@tok@gr\endcsname{\def\PYGdefault@tc##1{\textcolor[rgb]{1.00,0.00,0.00}{##1}}}
\expandafter\def\csname PYGdefault@tok@cm\endcsname{\let\PYGdefault@it=\textit\def\PYGdefault@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PYGdefault@tok@vg\endcsname{\def\PYGdefault@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PYGdefault@tok@m\endcsname{\def\PYGdefault@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PYGdefault@tok@mh\endcsname{\def\PYGdefault@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PYGdefault@tok@go\endcsname{\def\PYGdefault@tc##1{\textcolor[rgb]{0.53,0.53,0.53}{##1}}}
\expandafter\def\csname PYGdefault@tok@ge\endcsname{\let\PYGdefault@it=\textit}
\expandafter\def\csname PYGdefault@tok@vc\endcsname{\def\PYGdefault@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PYGdefault@tok@il\endcsname{\def\PYGdefault@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PYGdefault@tok@cs\endcsname{\let\PYGdefault@it=\textit\def\PYGdefault@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PYGdefault@tok@cp\endcsname{\def\PYGdefault@tc##1{\textcolor[rgb]{0.74,0.48,0.00}{##1}}}
\expandafter\def\csname PYGdefault@tok@gi\endcsname{\def\PYGdefault@tc##1{\textcolor[rgb]{0.00,0.63,0.00}{##1}}}
\expandafter\def\csname PYGdefault@tok@gh\endcsname{\let\PYGdefault@bf=\textbf\def\PYGdefault@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\expandafter\def\csname PYGdefault@tok@ni\endcsname{\let\PYGdefault@bf=\textbf\def\PYGdefault@tc##1{\textcolor[rgb]{0.60,0.60,0.60}{##1}}}
\expandafter\def\csname PYGdefault@tok@nl\endcsname{\def\PYGdefault@tc##1{\textcolor[rgb]{0.63,0.63,0.00}{##1}}}
\expandafter\def\csname PYGdefault@tok@nn\endcsname{\let\PYGdefault@bf=\textbf\def\PYGdefault@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PYGdefault@tok@no\endcsname{\def\PYGdefault@tc##1{\textcolor[rgb]{0.53,0.00,0.00}{##1}}}
\expandafter\def\csname PYGdefault@tok@na\endcsname{\def\PYGdefault@tc##1{\textcolor[rgb]{0.49,0.56,0.16}{##1}}}
\expandafter\def\csname PYGdefault@tok@nb\endcsname{\def\PYGdefault@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PYGdefault@tok@nc\endcsname{\let\PYGdefault@bf=\textbf\def\PYGdefault@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PYGdefault@tok@nd\endcsname{\def\PYGdefault@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\expandafter\def\csname PYGdefault@tok@ne\endcsname{\let\PYGdefault@bf=\textbf\def\PYGdefault@tc##1{\textcolor[rgb]{0.82,0.25,0.23}{##1}}}
\expandafter\def\csname PYGdefault@tok@nf\endcsname{\def\PYGdefault@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PYGdefault@tok@si\endcsname{\let\PYGdefault@bf=\textbf\def\PYGdefault@tc##1{\textcolor[rgb]{0.73,0.40,0.53}{##1}}}
\expandafter\def\csname PYGdefault@tok@s2\endcsname{\def\PYGdefault@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PYGdefault@tok@vi\endcsname{\def\PYGdefault@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PYGdefault@tok@nt\endcsname{\let\PYGdefault@bf=\textbf\def\PYGdefault@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PYGdefault@tok@nv\endcsname{\def\PYGdefault@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PYGdefault@tok@s1\endcsname{\def\PYGdefault@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PYGdefault@tok@sh\endcsname{\def\PYGdefault@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PYGdefault@tok@sc\endcsname{\def\PYGdefault@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PYGdefault@tok@sx\endcsname{\def\PYGdefault@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PYGdefault@tok@bp\endcsname{\def\PYGdefault@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PYGdefault@tok@c1\endcsname{\let\PYGdefault@it=\textit\def\PYGdefault@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PYGdefault@tok@kc\endcsname{\let\PYGdefault@bf=\textbf\def\PYGdefault@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PYGdefault@tok@c\endcsname{\let\PYGdefault@it=\textit\def\PYGdefault@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PYGdefault@tok@mf\endcsname{\def\PYGdefault@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PYGdefault@tok@err\endcsname{\def\PYGdefault@bc##1{\setlength{\fboxsep}{0pt}\fcolorbox[rgb]{1.00,0.00,0.00}{1,1,1}{\strut ##1}}}
\expandafter\def\csname PYGdefault@tok@kd\endcsname{\let\PYGdefault@bf=\textbf\def\PYGdefault@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PYGdefault@tok@ss\endcsname{\def\PYGdefault@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PYGdefault@tok@sr\endcsname{\def\PYGdefault@tc##1{\textcolor[rgb]{0.73,0.40,0.53}{##1}}}
\expandafter\def\csname PYGdefault@tok@mo\endcsname{\def\PYGdefault@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PYGdefault@tok@kn\endcsname{\let\PYGdefault@bf=\textbf\def\PYGdefault@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PYGdefault@tok@mi\endcsname{\def\PYGdefault@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PYGdefault@tok@gp\endcsname{\let\PYGdefault@bf=\textbf\def\PYGdefault@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\expandafter\def\csname PYGdefault@tok@o\endcsname{\def\PYGdefault@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PYGdefault@tok@kr\endcsname{\let\PYGdefault@bf=\textbf\def\PYGdefault@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PYGdefault@tok@s\endcsname{\def\PYGdefault@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PYGdefault@tok@kp\endcsname{\def\PYGdefault@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PYGdefault@tok@w\endcsname{\def\PYGdefault@tc##1{\textcolor[rgb]{0.73,0.73,0.73}{##1}}}
\expandafter\def\csname PYGdefault@tok@kt\endcsname{\def\PYGdefault@tc##1{\textcolor[rgb]{0.69,0.00,0.25}{##1}}}
\expandafter\def\csname PYGdefault@tok@ow\endcsname{\let\PYGdefault@bf=\textbf\def\PYGdefault@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\expandafter\def\csname PYGdefault@tok@sb\endcsname{\def\PYGdefault@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PYGdefault@tok@k\endcsname{\let\PYGdefault@bf=\textbf\def\PYGdefault@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PYGdefault@tok@se\endcsname{\let\PYGdefault@bf=\textbf\def\PYGdefault@tc##1{\textcolor[rgb]{0.73,0.40,0.13}{##1}}}
\expandafter\def\csname PYGdefault@tok@sd\endcsname{\let\PYGdefault@it=\textit\def\PYGdefault@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}

\def\PYGdefaultZbs{\char`\\}
\def\PYGdefaultZus{\char`\_}
\def\PYGdefaultZob{\char`\{}
\def\PYGdefaultZcb{\char`\}}
\def\PYGdefaultZca{\char`\^}
\def\PYGdefaultZam{\char`\&}
\def\PYGdefaultZlt{\char`\<}
\def\PYGdefaultZgt{\char`\>}
\def\PYGdefaultZsh{\char`\#}
\def\PYGdefaultZpc{\char`\%}
\def\PYGdefaultZdl{\char`\$}
\def\PYGdefaultZhy{\char`\-}
\def\PYGdefaultZsq{\char`\'}
\def\PYGdefaultZdq{\char`\"}
\def\PYGdefaultZti{\char`\~}
% for compatibility with earlier versions
\def\PYGdefaultZat{@}
\def\PYGdefaultZlb{[}
\def\PYGdefaultZrb{]}
\makeatother
\begin{SaveVerbatim}[commandchars=\\\{\}]{pytx@pycon@default@default@1}
\PYGdefault{g+gp}{\PYGdefaultZgt{}\PYGdefaultZgt{}\PYGdefaultZgt{} }\PYGdefault{k+kn}{import} \PYGdefault{n+nn}{Invasion\PYGdefaultZus{}PGF} \PYGdefault{k+kn}{as} \PYGdefault{n+nn}{pgf}
\PYGdefault{g+gp}{\PYGdefaultZgt{}\PYGdefaultZgt{}\PYGdefaultZgt{} }\PYGdefault{k}{def} \PYGdefault{n+nf}{mu}\PYGdefault{p}{(}\PYGdefault{n}{x}\PYGdefault{p}{)}\PYGdefault{p}{:}
\PYGdefault{g+gp}{... }    \PYGdefault{k}{return} \PYGdefault{p}{(}\PYGdefault{l+m+mi}{1} \PYGdefault{o}{+} \PYGdefault{n}{x} \PYGdefault{o}{+} \PYGdefault{n}{x}\PYGdefault{o}{*}\PYGdefault{o}{*}\PYGdefault{l+m+mi}{2} \PYGdefault{o}{+} \PYGdefault{n}{x}\PYGdefault{o}{*}\PYGdefault{o}{*}\PYGdefault{l+m+mi}{3}\PYGdefault{p}{)}\PYGdefault{o}{/}\PYGdefault{l+m+mf}{4.}
\PYGdefault{g+gp}{... }
\PYGdefault{g+gp}{\PYGdefaultZgt{}\PYGdefaultZgt{}\PYGdefaultZgt{} }\PYGdefault{n}{pgf}\PYGdefault{o}{.}\PYGdefault{n}{R0}\PYGdefault{p}{(}\PYGdefault{n}{mu}\PYGdefault{p}{)}
\PYGdefault{g+go}{1.5000001241105565}
\PYGdefault{g+gp}{\PYGdefaultZgt{}\PYGdefaultZgt{}\PYGdefaultZgt{} }\PYGdefault{c}{\PYGdefaultZsh{}extinction probabilities up to generation 5}
\PYGdefault{g+gp}{\PYGdefaultZgt{}\PYGdefaultZgt{}\PYGdefaultZgt{} }\PYGdefault{n}{pgf}\PYGdefault{o}{.}\PYGdefault{n}{extinction\PYGdefaultZus{}prob}\PYGdefault{p}{(}\PYGdefault{n}{mu}\PYGdefault{p}{,} \PYGdefault{l+m+mi}{5}\PYGdefault{p}{,} \PYGdefault{n}{intermediate\PYGdefaultZus{}values} \PYGdefault{o}{=} \PYGdefault{n+nb+bp}{True}\PYGdefault{p}{)}
\PYGdefault{g+go}{array([ 0.        ,  0.25      ,  0.33203125,  0.36972018,  0.38923784,}
\PYGdefault{g+go}{        0.39992896])}
\PYGdefault{g+gp}{\PYGdefaultZgt{}\PYGdefaultZgt{}\PYGdefaultZgt{} }\PYGdefault{c}{\PYGdefaultZsh{}following commands look at possible states in generation 3}
\PYGdefault{g+gp}{\PYGdefaultZgt{}\PYGdefaultZgt{}\PYGdefaultZgt{} }\PYGdefault{c}{\PYGdefaultZsh{}probability of 0..9 active infections in generation 3}
\PYGdefault{g+gp}{\PYGdefaultZgt{}\PYGdefaultZgt{}\PYGdefaultZgt{} }\PYGdefault{n}{pgf}\PYGdefault{o}{.}\PYGdefault{n}{active\PYGdefaultZus{}infections}\PYGdefault{p}{(}\PYGdefault{n}{mu}\PYGdefault{p}{,} \PYGdefault{l+m+mi}{3}\PYGdefault{p}{,} \PYGdefault{l+m+mi}{10}\PYGdefault{p}{)}
\PYGdefault{g+go}{array([ 0.36972018,  0.05259718,  0.07178445,  0.09609134,  0.07393309,}
\PYGdefault{g+go}{        0.07334027,  0.06617007,  0.05007252,  0.04119097,  0.03182213])}
\PYGdefault{g+gp}{\PYGdefaultZgt{}\PYGdefaultZgt{}\PYGdefaultZgt{} }\PYGdefault{c}{\PYGdefaultZsh{}probability of 0..9 completed infections in generation 3}
\PYGdefault{g+gp}{\PYGdefaultZgt{}\PYGdefaultZgt{}\PYGdefaultZgt{} }\PYGdefault{n}{pgf}\PYGdefault{o}{.}\PYGdefault{n}{completed\PYGdefaultZus{}infections}\PYGdefault{p}{(}\PYGdefault{n}{mu}\PYGdefault{p}{,} \PYGdefault{l+m+mi}{3}\PYGdefault{p}{,} \PYGdefault{l+m+mi}{10}\PYGdefault{p}{)}
\PYGdefault{g+go}{array([ \PYGdefaultZhy{}2.04281037e\PYGdefaultZhy{}17,   2.50000000e\PYGdefaultZhy{}01,   6.25000000e\PYGdefaultZhy{}02,}
\PYGdefault{g+go}{         7.81250000e\PYGdefaultZhy{}02,   9.76562500e\PYGdefaultZhy{}02,   1.21093750e\PYGdefaultZhy{}01,}
\PYGdefault{g+go}{         8.59375000e\PYGdefaultZhy{}02,   8.59375000e\PYGdefaultZhy{}02,   7.81250000e\PYGdefaultZhy{}02,}
\PYGdefault{g+go}{         6.25000000e\PYGdefaultZhy{}02])}
\PYGdefault{g+gp}{\PYGdefaultZgt{}\PYGdefaultZgt{}\PYGdefaultZgt{} }\PYGdefault{c}{\PYGdefaultZsh{}joint probabilities of 0..4 active infections and 0..4 completed}
\PYGdefault{g+gp}{\PYGdefaultZgt{}\PYGdefaultZgt{}\PYGdefaultZgt{} }\PYGdefault{c}{\PYGdefaultZsh{}infections in generation 3}
\PYGdefault{g+gp}{\PYGdefaultZgt{}\PYGdefaultZgt{}\PYGdefaultZgt{} }\PYGdefault{n}{pgf}\PYGdefault{o}{.}\PYGdefault{n}{active\PYGdefaultZus{}and\PYGdefaultZus{}completed}\PYGdefault{p}{(}\PYGdefault{n}{mu}\PYGdefault{p}{,} \PYGdefault{l+m+mi}{3}\PYGdefault{p}{,} \PYGdefault{l+m+mi}{5}\PYGdefault{p}{,} \PYGdefault{l+m+mi}{5}\PYGdefault{p}{)}
\PYGdefault{g+go}{array([[ 0.        ,  0.25      ,  0.0625    ,  0.03125   ,  0.015625  ],}
\PYGdefault{g+go}{       [ 0.        ,  0.        ,  0.        ,  0.015625  ,  0.015625  ],}
\PYGdefault{g+go}{       [ 0.        ,  0.        ,  0.        ,  0.015625  ,  0.01953125],}
\PYGdefault{g+go}{       [ 0.        ,  0.        ,  0.        ,  0.015625  ,  0.0234375 ],}
\PYGdefault{g+go}{       [ 0.        ,  0.        ,  0.        ,  0.        ,  0.01171875]])}
\PYGdefault{g+gp}{\PYGdefaultZgt{}\PYGdefaultZgt{}\PYGdefaultZgt{} }\PYGdefault{c}{\PYGdefaultZsh{}check that marginals match, increase sizes considered to improve match}
\PYGdefault{g+gp}{\PYGdefaultZgt{}\PYGdefaultZgt{}\PYGdefaultZgt{} }\PYGdefault{n}{act\PYGdefaultZus{}and\PYGdefaultZus{}complete} \PYGdefault{o}{=} \PYGdefault{n}{pgf}\PYGdefault{o}{.}\PYGdefault{n}{active\PYGdefaultZus{}and\PYGdefaultZus{}completed}\PYGdefault{p}{(}\PYGdefault{n}{mu}\PYGdefault{p}{,} \PYGdefault{l+m+mi}{3}\PYGdefault{p}{,} \PYGdefault{l+m+mi}{20}\PYGdefault{p}{,} \PYGdefault{l+m+mi}{20}\PYGdefault{p}{)}
\PYGdefault{g+gp}{\PYGdefaultZgt{}\PYGdefaultZgt{}\PYGdefaultZgt{} }\PYGdefault{n}{act\PYGdefaultZus{}and\PYGdefaultZus{}complete}\PYGdefault{o}{.}\PYGdefault{n}{sum}\PYGdefault{p}{(}\PYGdefault{n}{axis}\PYGdefault{o}{=}\PYGdefault{l+m+mi}{1}\PYGdefault{p}{)} \PYGdefault{c}{\PYGdefaultZsh{}Active infections}
\PYGdefault{g+go}{array([  3.69720176e\PYGdefaultZhy{}01,   5.25971800e\PYGdefaultZhy{}02,   7.17844516e\PYGdefaultZhy{}02,}
\PYGdefault{g+go}{         9.60913450e\PYGdefaultZhy{}02,   7.39330947e\PYGdefaultZhy{}02,   7.33402669e\PYGdefaultZhy{}02,}
\PYGdefault{g+go}{         6.61700666e\PYGdefaultZhy{}02,   5.00725210e\PYGdefaultZhy{}02,   4.11909670e\PYGdefaultZhy{}02,}
\PYGdefault{g+go}{         3.18221301e\PYGdefaultZhy{}02,   2.31783241e\PYGdefaultZhy{}02,   1.72899812e\PYGdefaultZhy{}02,}
\PYGdefault{g+go}{         1.21286511e\PYGdefaultZhy{}02,   8.08435678e\PYGdefaultZhy{}03,   5.25146723e\PYGdefaultZhy{}03,}
\PYGdefault{g+go}{         3.23349237e\PYGdefaultZhy{}03,   1.90655887e\PYGdefaultZhy{}03,   1.08598173e\PYGdefaultZhy{}03,}
\PYGdefault{g+go}{         5.83335757e\PYGdefaultZhy{}04,   2.96160579e\PYGdefaultZhy{}04])}
\PYGdefault{g+gp}{\PYGdefaultZgt{}\PYGdefaultZgt{}\PYGdefaultZgt{} }\PYGdefault{n}{act\PYGdefaultZus{}and\PYGdefaultZus{}complete}\PYGdefault{o}{.}\PYGdefault{n}{sum}\PYGdefault{p}{(}\PYGdefault{n}{axis}\PYGdefault{o}{=}\PYGdefault{l+m+mi}{0}\PYGdefault{p}{)} \PYGdefault{c}{\PYGdefaultZsh{}Completed infections}
\PYGdefault{g+go}{array([ 0.        ,  0.25      ,  0.0625    ,  0.078125  ,  0.09765625,}
\PYGdefault{g+go}{        0.12109375,  0.0859375 ,  0.0859375 ,  0.078125  ,  0.0625    ,}
\PYGdefault{g+go}{        0.0390625 ,  0.02342606,  0.01163167,  0.00376529,  0.        ,}
\PYGdefault{g+go}{        0.        ,  0.        ,  0.        ,  0.        ,  0.        ])}
\PYGdefault{g+gp}{\PYGdefaultZgt{}\PYGdefaultZgt{}\PYGdefaultZgt{} }\PYGdefault{c}{\PYGdefaultZsh{}yes, these match previous calculations, with a small mismatch because}
\PYGdefault{g+gp}{\PYGdefaultZgt{}\PYGdefaultZgt{}\PYGdefaultZgt{} }\PYGdefault{c}{\PYGdefaultZsh{}e.g., there may be 21 cumulative cases and 8 active cases.  To accurately}
\PYGdefault{g+gp}{\PYGdefaultZgt{}\PYGdefaultZgt{}\PYGdefaultZgt{} }\PYGdefault{c}{\PYGdefaultZsh{}calculate the probability of 8 active cases we would need to}
\PYGdefault{g+gp}{\PYGdefaultZgt{}\PYGdefaultZgt{}\PYGdefaultZgt{} }\PYGdefault{c}{\PYGdefaultZsh{}increase the sizes to include this.}

\PYGdefault{g+gp}{\PYGdefaultZgt{}\PYGdefaultZgt{}\PYGdefaultZgt{} }\PYGdefault{c}{\PYGdefaultZsh{}}
\PYGdefault{g+gp}{\PYGdefaultZgt{}\PYGdefaultZgt{}\PYGdefaultZgt{} }\PYGdefault{c}{\PYGdefaultZsh{}Now look at the final sizes}
\PYGdefault{g+gp}{\PYGdefaultZgt{}\PYGdefaultZgt{}\PYGdefaultZgt{} }\PYGdefault{n}{pgf}\PYGdefault{o}{.}\PYGdefault{n}{final\PYGdefaultZus{}sizes}\PYGdefault{p}{(}\PYGdefault{n}{mu}\PYGdefault{p}{,} \PYGdefault{l+m+mi}{20}\PYGdefault{p}{)}
\PYGdefault{g+go}{array([  0.00000000e+00,   2.50000000e\PYGdefaultZhy{}01,   5.93750000e\PYGdefaultZhy{}02,}
\PYGdefault{g+go}{         2.82031250e\PYGdefaultZhy{}02,   1.67456055e\PYGdefaultZhy{}02,   1.03404114e\PYGdefaultZhy{}02,}
\PYGdefault{g+go}{         6.80080902e\PYGdefaultZhy{}03,   4.66611063e\PYGdefaultZhy{}03,   3.29263648e\PYGdefaultZhy{}03,}
\PYGdefault{g+go}{         2.37637247e\PYGdefaultZhy{}03,   1.74605802e\PYGdefaultZhy{}03,   1.30159459e\PYGdefaultZhy{}03,}
\PYGdefault{g+go}{         9.81970183e\PYGdefaultZhy{}04,   7.48352208e\PYGdefaultZhy{}04,   5.75249662e\PYGdefaultZhy{}04,}
\PYGdefault{g+go}{         4.45491477e\PYGdefaultZhy{}04,   3.47250478e\PYGdefaultZhy{}04,   2.72225362e\PYGdefaultZhy{}04,}
\PYGdefault{g+go}{         2.14494366e\PYGdefaultZhy{}04,   1.69773210e\PYGdefaultZhy{}04])}
\PYGdefault{g+gp}{\PYGdefaultZgt{}\PYGdefaultZgt{}\PYGdefaultZgt{} }\PYGdefault{c}{\PYGdefaultZsh{}}
\PYGdefault{g+gp}{\PYGdefaultZgt{}\PYGdefaultZgt{}\PYGdefaultZgt{} }\PYGdefault{c}{\PYGdefaultZsh{}Now consider the continuous\PYGdefaultZhy{}time model}
\PYGdefault{g+gp}{\PYGdefaultZgt{}\PYGdefaultZgt{}\PYGdefaultZgt{} }\PYGdefault{n}{beta} \PYGdefault{o}{=} \PYGdefault{l+m+mi}{2}
\PYGdefault{g+gp}{\PYGdefaultZgt{}\PYGdefaultZgt{}\PYGdefaultZgt{} }\PYGdefault{n}{gamma} \PYGdefault{o}{=} \PYGdefault{l+m+mi}{1}
\PYGdefault{g+gp}{\PYGdefaultZgt{}\PYGdefaultZgt{}\PYGdefaultZgt{} }\PYGdefault{c}{\PYGdefaultZsh{}In next command, first returned array is the times and second}
\PYGdefault{g+gp}{\PYGdefaultZgt{}\PYGdefaultZgt{}\PYGdefaultZgt{} }\PYGdefault{c}{\PYGdefaultZsh{}is the extinction probabilities at those times}
\PYGdefault{g+gp}{\PYGdefaultZgt{}\PYGdefaultZgt{}\PYGdefaultZgt{} }\PYGdefault{n}{pgf}\PYGdefault{o}{.}\PYGdefault{n}{cts\PYGdefaultZus{}time\PYGdefaultZus{}extinction\PYGdefaultZus{}prob}\PYGdefault{p}{(}\PYGdefault{n}{beta}\PYGdefault{p}{,} \PYGdefault{n}{gamma}\PYGdefault{p}{,} \PYGdefault{l+m+mi}{5}\PYGdefault{p}{,} \PYGdefault{n}{intermediate\PYGdefaultZus{}values} \PYGdefault{o}{=}
\PYGdefault{g+gp}{... }                \PYGdefault{n+nb+bp}{True}\PYGdefault{p}{,} \PYGdefault{n}{numvals} \PYGdefault{o}{=} \PYGdefault{l+m+mi}{6}\PYGdefault{p}{)}
\PYGdefault{g+go}{(array([ 0.,  1.,  2.,  3.,  4.,  5.]),} 
\PYGdefault{g+go}{array([[ 0.        ,  0.38730017,  0.46371057,  0.48723549,  0.49537878,}
\PYGdefault{g+go}{         0.49830983]]))}
\PYGdefault{g+gp}{\PYGdefaultZgt{}\PYGdefaultZgt{}\PYGdefaultZgt{} }\PYGdefault{c}{\PYGdefaultZsh{}following commands look at possible states at time 3}
\PYGdefault{g+gp}{\PYGdefaultZgt{}\PYGdefaultZgt{}\PYGdefaultZgt{} }\PYGdefault{n}{pgf}\PYGdefault{o}{.}\PYGdefault{n}{cts\PYGdefaultZus{}time\PYGdefaultZus{}active\PYGdefaultZus{}infections}\PYGdefault{p}{(}\PYGdefault{n}{beta}\PYGdefault{p}{,} \PYGdefault{n}{gamma}\PYGdefault{p}{,} \PYGdefault{l+m+mi}{3}\PYGdefault{p}{,} \PYGdefault{l+m+mi}{10}\PYGdefault{p}{)}
\PYGdefault{g+go}{array([ 0.48723548,  0.01309038,  0.0127562 ,  0.01243055,  0.01211321,}
\PYGdefault{g+go}{        0.01180397,  0.01150263,  0.01120897,  0.01092282,  0.01064397])}
\PYGdefault{g+gp}{\PYGdefaultZgt{}\PYGdefaultZgt{}\PYGdefaultZgt{} }\PYGdefault{n}{pgf}\PYGdefault{o}{.}\PYGdefault{n}{cts\PYGdefaultZus{}time\PYGdefaultZus{}completed\PYGdefaultZus{}infections}\PYGdefault{p}{(}\PYGdefault{n}{beta}\PYGdefault{p}{,} \PYGdefault{n}{gamma}\PYGdefault{p}{,} \PYGdefault{l+m+mi}{3}\PYGdefault{p}{,} \PYGdefault{l+m+mi}{10}\PYGdefault{p}{)}
\PYGdefault{g+go}{array([ 0.00037014,  0.33477236,  0.07721546,  0.03805734,  0.02535527,}
\PYGdefault{g+go}{        0.02008499,  0.01755497,  0.0161637 ,  0.01527602,  0.0146211 ])}
\PYGdefault{g+gp}{\PYGdefaultZgt{}\PYGdefaultZgt{}\PYGdefaultZgt{} }\PYGdefault{c}{\PYGdefaultZsh{}check that the joint distribution has the same marginals}
\PYGdefault{g+gp}{\PYGdefaultZgt{}\PYGdefaultZgt{}\PYGdefaultZgt{} }\PYGdefault{n}{cts\PYGdefaultZus{}time\PYGdefaultZus{}act\PYGdefaultZus{}and\PYGdefaultZus{}complete} \PYGdefault{o}{=} \PYGdefault{n}{pgf}\PYGdefault{o}{.}\PYGdefault{n}{cts\PYGdefaultZus{}time\PYGdefaultZus{}active\PYGdefaultZus{}and\PYGdefaultZus{}completed}\PYGdefault{p}{(}\PYGdefault{n}{beta}\PYGdefault{p}{,} \PYGdefault{n}{gamma}\PYGdefault{p}{,} \PYGdefault{l+m+mi}{3}\PYGdefault{p}{,} \PYGdefault{l+m+mi}{20}\PYGdefault{p}{,} \PYGdefault{l+m+mi}{20}\PYGdefault{p}{)}
\PYGdefault{g+gp}{\PYGdefaultZgt{}\PYGdefaultZgt{}\PYGdefaultZgt{} }\PYGdefault{n}{cts\PYGdefaultZus{}time\PYGdefaultZus{}act\PYGdefaultZus{}and\PYGdefaultZus{}complete}\PYGdefault{o}{.}\PYGdefault{n}{sum}\PYGdefault{p}{(}\PYGdefault{n}{axis}\PYGdefault{o}{=}\PYGdefault{l+m+mi}{1}\PYGdefault{p}{)} \PYGdefault{c}{\PYGdefaultZsh{}Active infections}
\PYGdefault{g+go}{array([ 0.48717492,  0.01298644,  0.01257732,  0.0121518 ,  0.01170803,}
\PYGdefault{g+go}{        0.0112452 ,  0.01076355,  0.01026434,  0.00974976,  0.00922277,}
\PYGdefault{g+go}{        0.00868697,  0.00814639,  0.00760529,  0.00706802,  0.0065388 ,}
\PYGdefault{g+go}{        0.00602164,  0.00552019,  0.00503763,  0.00457669,  0.00413954])}
\PYGdefault{g+gp}{\PYGdefaultZgt{}\PYGdefaultZgt{}\PYGdefaultZgt{} }\PYGdefault{n}{cts\PYGdefaultZus{}time\PYGdefaultZus{}act\PYGdefaultZus{}and\PYGdefaultZus{}complete}\PYGdefault{o}{.}\PYGdefault{n}{sum}\PYGdefault{p}{(}\PYGdefault{n}{axis}\PYGdefault{o}{=}\PYGdefault{l+m+mi}{0}\PYGdefault{p}{)} \PYGdefault{c}{\PYGdefaultZsh{}Completed infections}
\PYGdefault{g+go}{array([ 0.00036997,  0.334771  ,  0.07720946,  0.03803859,  0.02530855,}
\PYGdefault{g+go}{        0.01998599,  0.0173696 ,  0.01584881,  0.0147816 ,  0.01389348,}
\PYGdefault{g+go}{        0.01306482,  0.01224544,  0.01141776,  0.01057991,  0.0097376 ,}
\PYGdefault{g+go}{        0.00889996,  0.00807718,  0.0072792 ,  0.00651487,  0.00579152])}
\PYGdefault{g+gp}{\PYGdefaultZgt{}\PYGdefaultZgt{}\PYGdefaultZgt{} }\PYGdefault{c}{\PYGdefaultZsh{}yes, these match previous calculations}
\PYGdefault{g+gp}{\PYGdefaultZgt{}\PYGdefaultZgt{}\PYGdefaultZgt{} }\PYGdefault{c}{\PYGdefaultZsh{}Now look at the final sizes at time infinity}
\PYGdefault{g+gp}{\PYGdefaultZgt{}\PYGdefaultZgt{}\PYGdefaultZgt{} }\PYGdefault{n}{pgf}\PYGdefault{o}{.}\PYGdefault{n}{cts\PYGdefaultZus{}time\PYGdefaultZus{}final\PYGdefaultZus{}sizes}\PYGdefault{p}{(}\PYGdefault{n}{beta}\PYGdefault{p}{,} \PYGdefault{n}{gamma}\PYGdefault{p}{,} \PYGdefault{l+m+mi}{20}\PYGdefault{p}{)}
\PYGdefault{g+go}{array([  0.00000000e+00,   3.33333333e\PYGdefaultZhy{}01,   7.40740741e\PYGdefaultZhy{}02,}
\PYGdefault{g+go}{         3.29218107e\PYGdefaultZhy{}02,   1.82898948e\PYGdefaultZhy{}02,   1.13803790e\PYGdefaultZhy{}02,}
\PYGdefault{g+go}{         7.58691934e\PYGdefaultZhy{}03,   5.29880081e\PYGdefaultZhy{}03,   3.82691169e\PYGdefaultZhy{}03,}
\PYGdefault{g+go}{         2.83474940e\PYGdefaultZhy{}03,   2.14181066e\PYGdefaultZhy{}03,   1.64421828e\PYGdefaultZhy{}03,}
\PYGdefault{g+go}{         1.27883644e\PYGdefaultZhy{}03,   1.00558079e\PYGdefaultZhy{}03,   7.98079995e\PYGdefaultZhy{}04,}
\PYGdefault{g+go}{         6.38463996e\PYGdefaultZhy{}04,   5.14318219e\PYGdefaultZhy{}04,   4.16833066e\PYGdefaultZhy{}04,}
\PYGdefault{g+go}{         3.39641758e\PYGdefaultZhy{}04,   2.78069275e\PYGdefaultZhy{}04])}
\end{SaveVerbatim}



==> solnfile.tex <==
\begin{solutionx}\solutionxparams 
\mbox{}
\begin{myenumerate}
\item Uniform: $p(\lambda)=1$, so the PGF is simply $0 + 0 + \cdots + 1 x^\lambda + 0 + 0 + \cdots = x^\lambda$.
\item Binomial: We have $r_i = \binom{n}{i} p^i q^{n-i}$.  So
\begin{align*}
\sum_i r_i x^i &= \sum_i \binom{n}{i} p^i q^{n-i}x^i\\
&= (px+q)^n
\end{align*}
by the binomial theorem.
\item Geometric: We have $r_i = q^ip$.  So
\begin{align*}
\sum_i r_i x^i &= \sum_i pq^ix^i\\
&= p \sum_i (qx)^i\\
&= \frac{p}{1-qx}
\end{align*}
by the sum of a geometric series.
\item Negative binomial: We have $r_i = \binom{i + \hat{r}-1}{i} q^{\hat{r}}p^i$.  So
\begin{align*}
\sum_i r_i x^i &= \sum_i \binom{i + \hat{r}-1}{i} q^{\hat{r}}p^ix^i\\
&= q^{\hat{r}} \sum_i \binom{i + \hat{r}-1}{i}p^i x^i\\
&=q^{\hat{r}}(1-px)^{-\hat{r}}\\
&= \left( \frac{q}{1-px}\right)^{\hat{r}}
\end{align*}
\end{myenumerate}
\end{solutionx}
\begin{solutionx}\solutionxparams 
We have $(px+q)^n$ where $p = \lambda/n$ and $q=1-p$.  Taking $n$ to be large gives
\begin{align*}
\lim_{n \to \infty} (q+px)^n &= \lim_{n\to\infty} \left( 1 + \frac{\lambda (x-1)}{n}\right)^n\\
&= e^{\lambda(x-1)}
\end{align*}
\end{solutionx}
\begin{solutionx}\solutionxparams 
\mbox{}
\begin{myenumerate}
\item In generation $0$ there is an infected individual.  So the disease is not extinct.  Thus $\alpha_0=0$.  If the outbreak is extinct at generation $g$, it remains extinct at later generations.  So $\alpha_g \leq \alpha_{g-1}$.  The eventual extinction probability is at most $1$.
\item Any sequence of numbers that is increasing and bounded from above must have a limit that is at most that bound.  So it converges to some limit $\alpha$.  Since $\mu(\alpha_g) = \alpha_{g+1}$, we conclude that $\mu(\alpha_g)$ must converge to the same limit.  Thus since $\mu$ is continuous, $\mu(\alpha)=\alpha$.
\item The assumptions of Property~\ref{property:PGFcobweb} hold, with $\Ro$ playing the role of $f'(1)$.  The property states that if $\Ro\leq 1$ the only solution is $\alpha=1$, while if $\Ro>1$ there is exactly one other solution in $(0,1)$.
\item The second part of Property~\ref{property:PGFcobweb} states that for $\Ro>1$, the solution must converge to this unique $\alpha<1$.  If $\Ro \leq 1$, the above observations show that it must converge to a solution to $\alpha = \mu(\alpha)$, and the only possible choice is $\alpha=1$.
\end{myenumerate}
\end{solutionx}
\begin{solutionx}\solutionxparams 
We only need the first two parts of Theorem~\ref{thm:strong_extinction}.  We have $\alpha = \lim_{g\to\infty}\alpha_g = \lim_{g\to\infty}\mu(\alpha_g)$.  Because $\mu$ is continuous we have $\lim_{g\to\infty} \mu(\alpha_g) = \mu(\lim_{g\to\infty}\alpha_g) = \mu(\alpha)$.

So $\alpha = \mu(\alpha)$.
\end{solutionx}
\begin{solutionx}\solutionxparams 
Let $\mu(0)=0$ and consider the smallest $g\geq 0$ such that $\alpha_{g+1} \neq 0$ (if it exists).  Then $\alpha_{g+1} = \mu(\alpha_g)=\mu(0)=0$.  So no such $g$ exists.

Biologically, $\mu(0)=0$ means that every individual has at least one offspring.  Thus if we start with one individual, we can never end up with zero.
\end{solutionx}
\begin{solutionx}\solutionxparams 
If $\mu(y) = \sum_{i=0}^\infty p_i x^i$ is a PGF and $\mu(0)=0$, then $p_0=0$ and $\mu(y) = \sum_{i=1}^\infty p_i x^i$ so $\Ro=\mu'(1) = \sum_{i=1}^\infty i p_i$.  This is $\geq \sum_{i=1}^\infty p_i=1$, with equality only if $p_i=0$ for $i>1$.  Thus the only such function is $\mu(y)=y$.

This corresponds to each individual having exactly one offspring.  So starting with one infection, at each generation there will remain exactly one infection, and there is no chance for extinction.  All other cases with $\Ro \leq 1$ have a nonzero chance of having zero offspring, and thus extinction is possible (and in fact inevitable).
\end{solutionx}
\begin{solutionx}\solutionxparams 
Let $\alpha$ be the extinction probability from one individual.
\begin{myenumerate}
\item The extinction probability given $m$ initial infections is $\alpha^m$.
\item Let $h(x) = \sum_m q_m x^m$.  The probability of extinction is $\sum_m q_m \alpha^m = h(\alpha)$.
\end{myenumerate}
\end{solutionx}
\begin{solutionx}\solutionxparams 
Define $\mu_1(y) = \sum_i p_i y^i = 0.1 + 0.2y + 0.65y^2+0.05y^3$.
\begin{myenumerate}
\item The extinction probability after $0$ generations is $\alpha_0=0$ and for $g>0$, the extinction probability after $g$ generations is $\alpha_g=\mu_1(\alpha_{g-1})$.  So by iteratively applying $\mu_1$ to $0$ we get
\begin{align*}
\alpha_0&=0\\
\alpha_1 &= \mu_1(\alpha_0) = 0.1\\
\alpha_2 &= \mu_1(\alpha_1) = 0.12655\\
\alpha_3 &= \mu_1(\alpha_2) \approx 0.13582\\
\alpha_4 &= \mu_1(\alpha_3) \approx 0.13928\\
\alpha_5 &= \mu_1(\alpha_4) \approx 0.14060
\end{align*}
\item Repeatedly applying $\mu_1$ to the result quickly yields convergence to $\alpha \approx 0.14143$.
\item Let $\mu_2(y) = 0.3+0.4y+0.3y^2$.  Assuming that there are still infected individuals when the intervention is introduced.  For each of them, the probability that all offspring die out is $\lim_{g\to\infty} \mu_2^{[g]}(0)\approx 0.9688$.

The distribution of the number infected when the intervention is introduced is $\mu_1(\mu_1(y))$.  So the probability of extinction is $\mu_1(\mu_1(0.9688)) \approx 0.9185$.
\end{myenumerate}
\end{solutionx}
\begin{solutionx}\solutionxparams 
\begin{myenumerate}
\item The PGF for the number infected in generation $g-1$ is
  $\Phi_{g-1}(y)$.  Each of the individuals who are infected in
  generation $g-1$ make some sort of contribution (possibly 0) to
  generation $g$.  The PGF for this contribution is $\mu(y)$.  Thus by
  Property~\ref{prop:composition}, the PGF for the combination of
  steps from generation $0$ to $g-1$ and from $g-1$ to $g$ is given by
  $\Phi_{g-1}(\mu(y))$.
\item The PGF for the number infected in generation $1$ is $\mu(y)$.
  If we trace the contributions of these individuals to generation
  $g$, we find that the distribution is the same as for the
  contribution of a generation $0$ individual to generation $g-1$.  So
  by Property~\ref{prop:composition}, the PGF for the  combination of steps from
  generation $0$ to $1$ and from $1$ to $g$ is $\mu(\Phi_{g-1}(y))$.
\end{myenumerate}
\end{solutionx}
\begin{solutionx}\solutionxparams 
The probability that there are no infections at generation $g$ is
given by $\Phi_g(0)$ (The expansion eliminates all terms except the
coefficient of $y^0$).

Simply observing $\Phi_g(0) = \mu^{[g]}(0)$ finishes the proof.
\end{solutionx}
\begin{solutionx}\solutionxparams 
The first part is simply multiplied by $k$.

For  $\langle I \rangle_g$, the numerator is multiplied by $k$.  The
denominator is the probability that the disease persists to generation
$g$.  This becomes $1-\alpha_g^k$.  This is because to be extinct, all $k$
introductions must independently go extinct, which occurs with
probability $\alpha_g^k$.
\end{solutionx}
\begin{solutionx}\solutionxparams 
\mbox{}
\begin{myenumerate}
\item Each individual causes 0, 1, or 2 transmissions with equal
  probability.
\item \begin{enumerate}
\renewcommand\labelenumii{(\roman{enumii})}
\renewcommand\theenumii\labelenumii
\item We have $\Omega_0(z)=1$ [there are no completed infections at generation $0$].
\item We have $\Omega_1(z)=z\mu(1) = z$ [which means that there is a single completed infection at generation $1$].
\item We have
\begin{align*}
\Omega_2(z)&= z\mu(\Omega_1(z))\\
&= z\mu(z)\\
&= \frac{z+z^2+z^3}{3}
\end{align*}
\item We have
\begin{align*}
\Omega_3(z) &= z \mu(\Omega_2(z))\\
&= z \frac{1+\Omega_2(z) + \Omega_2(z)^2}{3}\\
&= \frac{9z + 3z^2 + 4 z^3  + 5 z^4+ 3z^5 + 2 z^6 +z^7 }{27}\\
&= \frac{z}{3} + \frac{z^2}{9} + \cdots
\end{align*}
\item and finally
\begin{align*}
\Omega_4(z) &= z\mu(\Omega_3(z))\\
&= z \frac{1+\Omega_3(z) + \Omega_3(z)^2 + }{3}\\
&=
\frac{1}{2187} \big(729z  + 243z^2 + 162 z^3 +  162 z^4 +  216 z^5 +
  105 z^6 +  154 z^7\\
&\qquad\qquad +  121 z^8 +  79 z^9 +  52 z^{10} +  37 z^{11} +  22 z^{12} +  10 z^{13} +  4 z^{14} +  z^{15}\big)\\
&= \frac{z}{3} + \frac{z^2}{9} + \cdots
\end{align*}
\end{enumerate}
\item
\begin{itemize}
\item For $r=0$, we see that from $\Omega_1(z)$ onwards, the coefficient of $z^0$ is $0$.
\item For $r=1$, we see that from $\Omega_2(z)$ onwards, the coefficient of $z$ is $1/3$
\item For $r=2$, we see that from $\Omega_3(z)$ onwards, the coefficient of $z^2$ is $1/9$.
\end{itemize}
\end{myenumerate}
\end{solutionx}
\begin{solutionx}\solutionxparams 
We expect that $\Pi_g(1,z) = \Omega(z)$.  This can be checked by
noting that for given $r$, the sum $\sum_i \pi_{i,r}(g) 1^i z^r$ is
$z^r \sum_i \pi_{i,r}(g) = z^r\omega_r(g)$.

So Theorem~\ref{thm:joint_size} states that $\Pi_g(1,z) = z
\mu(\Pi_{g-1}(1,z))$ which becomes $\Omega_g(z) = z \mu(\Omega_{g-1}(z))$.
\end{solutionx}
\begin{solutionx}\solutionxparams 
The key observation is that $\hat{r}j(\hat{r}j+1) \cdots (\hat{r}j + j
- 2)/(j-1)!$ becomes $\Gamma(\hat{r}j+j-1)/\Gamma(\hat{r}j-1)
(j-1)!$.  Thus we replace $\binom{\hat{r}j + j -2}{j-1}$ in the
expression to yield
\[
\frac{1}{j} \frac{\Gamma(\hat{r}j+j-2)}{\Gamma(\hat{r}j-1)(j-1)!}
q^{\hat{r}j} p^{j-1}
\]
\end{solutionx}
\begin{solutionx}\solutionxparams 
For each we need to find the coefficient of $y^{j-1}$ in $[\mu(y)]^j$ and then divide it by $j$.
\begin{myenumerate}
\item $[\mu(y)]^j = e^{j\lambda(y-1)}$  The coefficient of $y^{j-1}$ is
\begin{align*}
\left. \frac{1}{(j-1)!} \left(\diff{}{y}\right)^{j-1} e^{j\lambda(y-1)}\right|_{y=0} &= \left. \frac{1}{j-1} (j\lambda)^{j-1} e^{j\lambda(y-1)} \right|_{y=0}\\
&= \frac{(j\lambda)^{j-1}}{(j-1)!} e^{-\lambda j}
\end{align*}
Taking $1/j$ times this yields $\frac{(\lambda j)^{j-1}}{j!} e^{-\lambda j}$.
\item Note that for this to make sense $\lambda$ must be a non-negative integer.  We have $[\mu(y)]^j = y^{\lambda j}$.  The first case we consider is $j=1$, \ $\lambda = 0$.  Then we have $[\mu(y)]^j = 1$.  Taking zero derivatives, setting $y=0$, and dividing by $(j-1)! =1$ and $j=1$ yields $1$.

Now consider $\lambda\geq 1$.  Then $\lambda j>j-1$.  So after taking $j-1$ derivatives, we still have a factor of $y$, which when we set $y=0$ yields $0$.

Now consider $\lambda = 0$, but $j>1$.  We have $[\mu(y)]^j = 1$.  Taking $j-1\geq 1$ derivatives yields $0$.

\item We have $[\mu(y)]^j = (q+py)^{jn}$.  By the binomial theorem, the coefficient of $y^{j-1}$ is $\binom{jn}{j-1} q^{jn-j+1}p^{j-1}$.  Taking $1/j$ times this yields the result
\item We have $[\mu(y)]^j = \left(p/(1-qy)\right)^j$.  Following the same steps as in the negative binomial distribution, but taking $\hat{r}=1$ and interchanging $p$ and $q$, we end up with $\frac{1}{j} \binom{2j-2}{j-1} p^jq^{j-1}$.
\end{myenumerate}
\end{solutionx}
\begin{solutionx}\solutionxparams 
\mbox{}
\begin{myenumerate}
\item After a generation, an individual contributes $\mu(y)$ new
  infections and $1$ new recovery.  This is captured by $\mu(y,z) = z \mu(y)$.
\item $\Omega_g(z) = \mu(\Omega_{g-1}(z),z)$.
\item $\Pi_g(y,z) = \mu(\Pi_{g-1}(y,z),z)$.
\end{myenumerate}
\end{solutionx}
\begin{solutionx}\solutionxparams 
\mbox{}
\begin{myenumerate}
\item There are now three observations $j=7$, \ $j=8$, and $j=4$.
  Adapting the result in the example, we
  have
\[
f(\Theta) = \left(\sum_{j=7,8,4} \log ((\hat{r}j+j-2)!) - \log(j!) - \log
  ((\hat{r}j-1)!) +\hat{r}j \log q + (j-1) \log p\right) + \log 0.5 \, .
\]
We find $f(\Theta_1) \approx  -11.3978$ and $f(\Theta_2) \approx -12.0858$.  So
$\hat{f}(\Theta_1) =0$ and $\hat{f}(\Theta_2) = -0.688$.  Then
$g(\Theta_1) = 1$ and $g(\Theta_2) = 0.5026$.  We finally have
\[
P(\Theta_1|X) = 0.6655 , \qquad P(\Theta_2|X) = 0.3345
\]
\item The difference appears at the beginning:
\[
f(\Theta_1) = \left(\log ((\hat{r}4+4-2)!) - \log(4!) - \log
  ((\hat{r}4-1)!) +\hat{r}4 \log q + (4-1) \log p\right) + \log 0.6546
\]
and
\[
f(\Theta_2) = \left(\log ((\hat{r}4+4-2)!) - \log(4!) - \log
  ((\hat{r}4-1)!) +\hat{r}4 \log q + (4-1) \log p\right) + \log 0.3454
\, .
\]
Plugging in for $\hat{r}$, we get  $f(\Theta_1) = -3.326$
and $f(\Theta_2) = -4.014$.  Once we find $\hat{f}$ we find that it
takes the same value as in the previous part, and so the results follow.

\item If we update our beliefs with all of our observations, we should
  get the same final outcome.  This should depend on whether we do it
  all at once, or sequentially (or even what order we do it
  sequentially).
\end{myenumerate}
\end{solutionx}
\begin{solutionx}\solutionxparams 
The PGF is $\left( \frac{0.98}{1-0.02x}\right)^{\hat{r}}$.  We start
off with $P(\Theta) = 1/80$ for all integers from $1$ to $80$.  Given
$\hat{r}$ and $p=0.02$, the probability of observing a particular size
$j$ is $\frac{1}{j} \binom{\hat{r} j + j-2}{j-1} 0.98^{\hat{r}j}
0.01^{j-1}$.


\begin{myenumerate}
\item So $P(X|\Theta)$ means the probability of observing sizes $1$, $4$,
  $5$, $6$, and $10$ in five outbreaks given the value $\hat{r}$.
  For simplicity, we note that $1\cdot 4\cdot 5 \cdot 6 \cdot 10
  =1200$ and $1+ 4+ 5 + 6 + 10 = 26$ This is
\[
P(1,4,5,6,10 | \hat{r}) = \frac{1}{1200} 0.98^{26 \hat{r}}0.02^{26-5}
\binom{\hat{r}-1}{0} \binom{4\hat{r} + 2}{3}\binom{5\hat{r}+3}{4}\binom{6\hat{r}+4}{5}\binom{10\hat{r}+8}{9}
\]
Following the steps we get
\raisebox{-0.5\height}{\includegraphics[width=0.5\textwidth]{infplt.pdf}}
\item By summing the probabilities over all $\hat{r}$ for which $\Ro>1$, we find the
  probability that $\Ro>1$ is 0.181
\end{myenumerate}
\end{solutionx}
\begin{solutionx}\solutionxparams 
\mbox{}
\begin{myenumerate}
\item $y(\beta+\gamma) = \beta y^2 + \gamma$ so
\[
\beta y^2 - (\beta+ \gamma)y + \gamma = 0
\]
By the quadratic formula
\[
y = \frac{\beta+\gamma \pm \sqrt{(\beta+\gamma)^2 -
    4\beta\gamma}}{2\beta}
\]
The radical becomes $\sqrt{\beta^2 - 2\beta\gamma +\gamma^2} =
(\beta-\gamma)$.
So
\[
y = \frac{\beta+\gamma \pm (\beta-\gamma)}{2\beta} = \{ 1, \gamma/\beta\}
\].
\item If $\beta < \gamma$, then only $1$ is in the interval.
\item If $\gamma>\beta$ then both are in the interval.
\end{myenumerate}
\end{solutionx}
\begin{solutionx}\solutionxparams 
\mbox{}
\begin{myenumerate}
\item The event is either a recovery or a transmission, and the rates
  are $\gamma$ and $\beta$.  So the probability of recovery is the
  rate of recovery divided by the total rate.
\item While the individual is susceptible, the probability that the
  next event is a transmission is $\beta/(\beta+\gamma)$.  So the
  probability that the first $i$ events are transmissions is
  $\beta^i/(\beta+\gamma)^i$.  The probability that the next event is
  a recovery is $\gamma/(\beta+\gamma)$.  The product of these is the
  probability that the first $i$ events are transmissions and the next
  event is a recovery.
\item Let $r = \beta/(\beta+\gamma)$.  Then $p_i = (1-r) r^i$.  Then $\sum_ip_i y^i$ is a geometric series: $(1-r) \sum_i (ry)^i = (1-r)/(1-ry)$.  Multiplying by $1=(\beta+\gamma)/(\beta+\gamma)$ gives the result.
%\item Explain why $\mu(y)$ corresponds to a  geometric distribution
%(see Table~\ref{tab:example_PGFs}).
\item The solutions to $y = \mu(y)$ are the solutions to
  $y(\beta+\gamma-\beta y) = \gamma$.  The solutions to $y =
  \hat{\mu}(y) = (\beta y^2+\gamma)/(\beta+\gamma)$ are the solutions
  to $y(\beta+\gamma) = \beta y^2 + \gamma$.  By moving $\beta y^2$ to
  the other side of either equation we see that the equations are
  equivalent.
\end{myenumerate}
\end{solutionx}
\begin{solutionx}\solutionxparams 
 \mbox{}
\begin{myenumerate}
\item $\mu'(y) = \gamma \beta/(\beta+\gamma-\beta y)^2$, so $\mu'(1) = \gamma\beta/\gamma^2 = \beta/\gamma$.  Similarly $\hat{\mu}'(y) = 2\gamma y/(\beta+\gamma)$, so $\hat{\mu}'(1) = 2\gamma/(\beta+\gamma)$.  These are generally unequal.
\item When $\Ro = 1$, we have $\beta = \gamma$.  So $\mu'(1) = \gamma/\gamma=1$ and $\hat{\mu}'(1) = 2\gamma/(\gamma+\gamma)=1$.  So the two are equal.
\end{myenumerate}
\end{solutionx}
\begin{solutionx}\solutionxparams 
\mbox{}
\begin{myenumerate}
\item We have
\begin{align*}
\dot{\alpha} &= (\beta+\gamma)\left(\frac{\beta \alpha^2+ \gamma}{\beta+\gamma}-\alpha\right)\\
&= \beta \alpha^2 + \gamma  - \alpha\\
&= (1-\alpha)(\gamma-\beta \alpha)
\end{align*}
\end{myenumerate}
Starting from $\alpha(0)=0$, we see that $\dot{\alpha}(0) =\gamma >0$.  So $\alpha$ will increase and approach the smallest positive equilibrium value. The two equilibria are at $\alpha=1$ and $\alpha = \gamma/\beta$.
\begin{continuemyenumerate}
\item If $\beta<\gamma$, then the smaller equilibrium is $\alpha=1$.
\item If $\beta>\gamma$, then the smaller equilibrium is $\alpha = \gamma/\beta$.
\item We have
\[
\frac{\diff{\alpha}{t}}{(1-\alpha)(\gamma-\beta\alpha)} = 1
\]
So using separation of variables, we have
\[
\int \frac{1}{(1-\alpha)(\gamma-\beta\alpha)} \, \mathrm{d}\alpha = \int 1 \mathrm{d}t
\]
Using partial fractions this becomes
\[
\int \frac{A}{1-\alpha} + \frac{B}{\gamma-\beta \alpha} \, \mathrm{d}\alpha = \int 1 \, \mathrm{d}t
\]
where $A$ and $B$ are chosen such that the sum in the integrand has a
numerator of $1$.  Once $A$ and $B$ are found, both sides can be integrated analytically.
\end{continuemyenumerate}
\end{solutionx}
\begin{solutionx}\solutionxparams 
\mbox{}
\begin{myenumerate}
\item We have
\begin{align*}
\phi_0(\Delta t) &= \gamma \Delta t + \littleo(\Delta t)\\
\phi_1(\Delta t) &= 1- (\beta+\gamma) \Delta t + \littleo(\Delta t)\\
\phi_2(\Delta t) &= \beta \Delta t + \littleo(\Delta t)
\end{align*}
\item If the disease is extinct at time $\Delta t$, then it remains extinct.
\item This equals the probability of having $1$ infection at time $t_0$ if there is one infection at time $0$.  So it is is $\phi_1(t_0)$.
\item One of the infections has to have its descendants go extinct within $t_0$ units of time, and the other must have 1 descendant after $t_0$ units of time.  So this is $\phi_0(t_0)\phi_1(t_0) + \phi_1(t_0)\phi_0(t_0) = 2\phi_0(t_0) \phi_1(t_0)$
\item So  [using the additional fact that the probability of 3 or more infections at time $\Delta t$ is $\littleo(\Delta t)$]
\[
\phi_1(t_0+\Delta t) = \phi_1(\Delta t)\phi_1(t_0) + 2\phi_2(\Delta t)\phi_0(t_0)\phi_1(t_0) + \littleo(\Delta t)
\]
\item So
\begin{align*}
\dot{\phi}_1(t) &= \lim_{\Delta t \to 0} \frac{\phi_1(t+\Delta t) - \phi_1(t)}{\Delta t}\\
&= \lim_{\Delta t \to 0} \frac{\phi_1(\Delta t)\phi_1(t) + 2\phi_2(\Delta t)\phi_0(t)\phi_1(t) + \littleo(\Delta t) - \phi_1(t)}{\Delta t}\\
&= \lim_{\Delta t \to 0} \frac{[1-(\beta+\gamma)\Delta t] \phi_1(t) + 2\beta \Delta t\phi_0(t)\phi_1(t) + \littleo(\Delta t) - \phi_1(t)}{\Delta t}\\
&= \lim_{\Delta t \to 0} \frac{-(\beta+\gamma)\Delta t \phi_1(t) + 2\beta \Delta t\phi_0(t)\phi_1(t) + \littleo(\Delta t)}{\Delta t}]\\
&= -(\beta+\gamma)\phi_1(t) + 2\beta \phi_0(t)\phi_1(t)
\end{align*}
\end{myenumerate}
\end{solutionx}
\begin{solutionx}\solutionxparams 
\mbox{}
\begin{myenumerate}
\item If there are $j$ infected individuals, then a new transmission will result in $j+1$ total infections and occurs at total rate $\beta j$.  This appears as a loss to $\phi_j$ at rate $j\beta \phi_j$, but a gain at rate $(j-1)\beta\phi_{j-1}$ from the smaller state.
Similarly a recovery will result in $j-1$ total infections and occurs at total rate $\gamma j$.  No other possibilities are considered in our model.   This appears as a loss at rate $j \gamma \phi_j$ and a gain at rate $(j+1)\gamma \phi_{j+1}$.
\item
We convert this into an equation for the PGF:
\begin{align*}
\pd{}{t} \Phi(y,t) &=\pd{}{t} \sum_j \phi_j(t) y^j \\
&= \sum_j \dot{\phi}_j(t) y^j\\
&= \sum_j \beta(j-1)\phi_{j-1}y^j + \gamma(j+1)\phi_{j+1}y^j-(\beta+\gamma)j \phi_j y^j\\
&=  \beta \sum_j (y^2-y)\pd{}{y} \phi_{j-1}y^{j-1}  + \gamma \sum_j \pd{}{y} \phi_{j+1}y^{j+1} - (\beta+\gamma) \sum_j y \pd{}{y} \phi_j y^j\\
&=[\beta(y^2-y) +\gamma - (\beta+\gamma)y\pd{}{y}\Phi(y,t)\\
&= (\beta+\gamma)\left[\hat{\mu}(y) - y \right] \pd{}{y}\Phi(y,t)
\end{align*}
\end{myenumerate}
\end{solutionx}
\begin{solutionx}\solutionxparams 
\mbox{}
\begin{myenumerate}
\item If $\Delta t$ is very small then to leading order either $0$ or $1$ event occurs in the first $\Delta t$ units of time
\begin{itemize}
\item The probability of $0$ events if we start with $k$ infections is $1-k(\beta+\gamma)\Delta t + \littleo(\Delta t) $.  In this case the probability of $i$ infections at time $t+\Delta t$ is the same as the probability of $i$ infections at time $t$ given the initial condition.
\item The probability of $1$ event occurring and it being an infection is $k\beta \Delta t + \littleo(\Delta t)$.  In this the probability of $i$ infections at time $t+\Delta t$ is the same as the probability of $i$ infections at time $t$ if we start with $k+1$ infections, $\phi_{(k+1)i}$.
\item The probability of 1 event occurring and it being a recovery is $k \gamma \Delta t + \littleo(\Delta t)$.  Following the previous case, this corresponds to starting with $k-1$ infections, $\phi_{(k-1)i}$.
\end{itemize}
Adding these together gives the result.
\item \[
\dot{\phi}_{ki} = -k(\beta+\gamma)\phi_{ki} + k\beta \phi_{(k+1)i} + k\gamma \phi_{(k-1)i}
\]
\item
\begin{align*}
\dot{\Phi}(y, t | 1) &= \sum_i\dot{\phi}_{1i}y^i\\
&= \sum_i -(\beta+\gamma)\phi_{1i}y^i + \beta \phi_{2i}y^i+\gamma\phi_{0i}y^i\\
&= - (\beta+\gamma) \Phi(y,t|1) + \beta \Phi(y,t|2) + \gamma \Phi(y,t|0)
\end{align*}
\item This follows from $k$ applications of Property~\ref{property:sum2product}.
\item So we use $\Phi(y,t|2)=\Phi(y,t|1)^2$ and $\Phi(y,t|0)=1$ to give
\begin{align*}
\dot{\Phi}(y,t|1) &= -(\beta+\gamma)\Phi(y,t|1)+ \beta \Phi(y,t|1)^2 + \gamma\\
&= (\beta+\gamma) \left[ \frac{\beta \Phi(y,t|1)^2 + \gamma}{\beta+\gamma} - \Phi(y,t|1) \right]\\
&= (\beta+\gamma) [\hat{\mu(\Phi(y,t|1))} - \Phi(y,t|1)]
\end{align*}
Replacing $\Phi(y,t|1)$ with $\Phi(y,t)$ completes the derivation.
\end{myenumerate}
\end{solutionx}
\begin{solutionx}\solutionxparams 
\mbox{}
\begin{myenumerate}
\item This follows from $k$ applications of Property~\ref{property:sum2product}.
\item On the left hand side, the substitution yields
\[
\pd{}{t} \Phi(y,t)^k = k \Phi(y,t)^{k-1} \pd{}{t} \Phi(y,t)
\]
and on the right hand side we get
\[
  (\beta+\gamma) [\hat{\mu}(y) - y] \pd{}{y} \Phi(y,t)^k = k \Phi(y,t)^{k-1} (\beta+\gamma) [\hat{\mu}(y) - y] \pd{}{y} \Phi(y,t)
\]
The $k \Phi(y,t)^{k-1}$ term on each side cancel, and we have a correct equation.
\item On the left hand side the substitution yields
\[
\pd{}{t} \Phi(y,t)^k = k \Phi(y,t)^{k-1} \pd{}{t} \Phi(y,t)
\]
as before, but on the right hand side we get
\[
(\beta+\gamma) [\hat{\mu}(\Phi(y,t)^k) - \Phi(y,t)^k]
= \beta\Phi(y,t)^{2k} + \gamma - (\beta+\gamma)\Phi(y,t)^k
\]
There is no common term we can cancel to get back to the original equation.
\end{myenumerate}
\end{solutionx}
\begin{solutionx}\solutionxparams 
We have
\begin{align*}
\dot{\Phi}(y, t | k ) &= \sum_i \dot{\phi}_{ki} y^i\\
&= \sum_i\left[ -k (\beta+\gamma) \phi_{ki} + k\beta \phi_{(k+1)i} + k\gamma
  \phi_{(k-1)i} \right]y^i\\
&= -k(\beta+\gamma)  \Phi(y, t |k)  + k \beta \Phi(y, t| k+1) + k
  \gamma \Phi(y, t | k-1)
\end{align*}
\end{solutionx}
\begin{solutionx}\solutionxparams 
\mbox{}
\begin{myenumerate}
\item We know that $\alpha(0)=0$. Substituting into Equation~\eqref{eqn:forward_PGF}
\begin{align*}
\dot{\alpha}(t) &= (\beta+\gamma) [\hat{\mu}(0)-0] \pd{}{y} \Phi(0,t)\\
&= \gamma \pd{}{y} \Phi(0,t)\\
&= \gamma \phi_1(t)
\end{align*}
We would also need to know the probability of having one infection at any given time.
\item Again, we know that $\alpha(0)=0$.  Substituting into Equation~\eqref{eqn:backward_PGF} yields
\[
\dot{\alpha} = (\beta+\gamma) [\hat{\mu}(\alpha) - \alpha]
\]
We would not need any additional information to solve this
\end{myenumerate}
\end{solutionx}
\begin{solutionx}\solutionxparams 
\mbox{}
\begin{myenumerate}
\item If we substitute for $\hat{\mu}$, we get
\begin{align*}
\pd{}{t} \Phi(y,t) &= (\beta+\gamma) \left( \frac{\beta [\Phi(y,t)]^2 +
    \gamma}{\beta+\gamma}  - \Phi(y,t)\right)\\
&= \beta[\Phi(y,t)]^2 + \gamma - (\beta+\gamma)\Phi(y,t)
\end{align*}
and
\begin{align*}
(\gamma-\beta \Phi(y,t) ) (1-\Phi(y,t)) &= \gamma - \gamma\Phi(y,t) -
                                          \beta\Phi(y,t) + \beta[\Phi(y,t)]^2\\
&=  \beta [\Phi(y,t)]^2 - (\beta+\gamma)\Phi(y,t) + \gamma
\end{align*}
So these are equal.
\item We have
\[
\int \frac{1}{(\gamma - \beta \Phi(y,t)) (1-\Phi(y,t))}
\mathrm{d}\Phi(y,t) = \int \mathrm{d}t
\]
We write the first integrand as $ \frac{1}{(\gamma - \beta \Phi(y,t)) (1-\Phi(y,t))}=\frac{A}{\gamma-\beta\Phi(y,t)} +
\frac{B}{1-\Phi(y,t)}$ and must solve for $A$ and $B$.  Then this is integrable.
\end{myenumerate}
\end{solutionx}
\begin{solutionx}\solutionxparams 
We have $\Phi(y,t) = \sum_i \phi_i(t) y^i$ where $\phi_i(t)$ is the
probability of $i$ infections at time $t$.  Similarly
\begin{align*}
\Pi(y,z,t)|_{z=1} &= \left.\sum_{i,r} \pi_{i,r} y^i z^r \right|_{z=1}\\
&= \sum_{i}\sum_r  \pi_{i,r} y^i1^r\\
&= \sum_i \left(y^i \sum_r \pi_{i,r}\right)
\end{align*}
and because $\sum_r \pi_{i,r} = \phi_i$, the result follows.
\end{solutionx}
\begin{solutionx}\solutionxparams 
Note that $\Phi(y,t) = \Pi(y,1,t)$.  Setting $z=1$ into the equation for $\Pi$ yields the equation for $\Phi$.
\end{solutionx}
\begin{solutionx}\solutionxparams 
Note that for $z<1$, \ $\Omega_\infty(z) = \lim_{t \to \infty}
\Pi(0,z,t)$ and for $z=1$ it is $1$.

As $t \to \infty$, we must have $\pd{}{t} Pi(0,z,t) = 0$ since the
system approaches a disease-free state and thus all coefficients
converge to a constant.  For this to hold,
Equation~\eqref{eqn:backward_result} yields
\[
\lim_{t\to\infty} \hat{\mu}(\Pi(0,z,t), z) = \lim_{t\to\infty}\Pi(0, z, t)
\]
Substituting with $\Omega_\infty$ completes the result.

\end{solutionx}
\begin{solutionx}\solutionxparams 
We take
\begin{align*}
\Omega_\infty(z) &= \hat{\mu}(\Omega_\infty(z), z)\\
&= \frac{\beta [\Omega_\infty(z)]^2 + \gamma z}{\beta+\gamma}
\end{align*}
So
\begin{align*}
(\beta+\gamma) \Omega_\infty(z) &= \beta [\Omega_\infty(z)]^2 + \gamma
                                  z\\
\Omega_\infty(z)[\beta+\gamma - \beta \Omega_\infty(z)]  &= \gamma z\\
\Omega_\infty(z) & = \frac{\gamma z}{\beta+\gamma-\beta\Omega_\infty(z)}
\end{align*}
\end{solutionx}
\begin{solutionx}\solutionxparams 
\mbox{}
\begin{myenumerate}
\item We have
\begin{align*}
[\dot{S}] &= \left . \pd{}{t} \pd{}{x} \Xi(x,y,t)\right|_{x=y=1}\\
& = \left . \pd{}{x} \pd{}{t} \Xi(x,y,t)\right|_{x=y=1}\\
&= \left . \pd{}{x}\left( \frac{\beta(y^2-xy)}{N}\pd{}{x}\pd{}{y}\Xi(x,y,t) +
  \gamma(1-y) \pd{}{y} \Xi(x,y,t) \right)\right |_{x=y=1}\\
&= \left. -\frac{\beta y}{N} \pd{}{x}\pd{}{y} \Xi(x,y,t)  +
  \frac{\beta(y^2-xy)}{N}\pds{}{x} \pd{}{y} \Xi(x,y,t) + \gamma (1-y)
  \pd{}{x}\pd{}{y} \Xi(x,y,t) \right|_{x=y=1}\\
&= - \frac{\beta}{N} \pd{}{x}\pd{}{y} \Xi(1,1,t)\\
&= - \frac{\beta}{N} [SI]
\end{align*}
\item We have
\begin{align*}
[\dot{I}] &= \left . \pd{}{t} \pd{}{y} \Xi(x,y,t) \right|_{x=y=1}\\
&= \left . \pd{}{y} \left( \frac{\beta(y^2-xy)}{N}\pd{}{x}\pd{}{y}\Xi(x,y,t) +
  \gamma(1-y) \pd{}{y} \Xi(x,y,t) \right)\right |_{x=y=1}\\
&= \left. \frac{\beta(2 y - x)}{N} \pd{}{x}\pd{}{y} \Xi(x,y,t) +
  \frac{\beta(y^2-xy)}{N}\pd{}{x}\pds{}{y} \Xi(x,y,t) - \gamma
  \pd{}{y} \Xi(x,y,t) + \gamma(1-y)\pds{}{y} \Xi(x,y,t)
  \right|_{x=y=1}\\
&=\frac{\beta}{N} \pd{}{x}\pd{}{y} \Xi(1,1,t)  - \gamma
  \pd{}{y}\Xi(1,1,t)\\
&= \frac{\beta}{N} [SI] - \gamma [I]
\end{align*}
\item As $[\dot{S}] + [\dot{I}] + [\dot{R}] = 0$, we conclude
\[
[\dot{R}] = -[\dot{S}] - [\dot{I}] = \gamma [I]
\]
\end{myenumerate}
\end{solutionx}
\begin{solutionx}\solutionxparams 
\mbox{}
\begin{myenumerate}
\item From Graph Theory, the average in-degree must equal the average
  out-degree.

Alternately we can note that the average number of
  edges coming out of a node is the total number of edges divided by
  $N$, so the total number of edges is expected to be $\Ro N$.  Then
  the average number of edges in is also the total number divided by
  $N$, that is, $\Ro$.
\item Individual $v$ receives a given transmission with probability
  $1/N$.  There are $\Ro N$ edges, each of which could reach $v$ with
  probability $1/N$.  So this defines a binomial distribution.
\item As $N$ increases, the probability a particular edge goes to $v$
  is $1/N$, while the number of edges is $\Ro N$.  This defines a
  Poisson distribution with mean $\Ro$.
\end{myenumerate}
\end{solutionx}
\begin{solutionx}\solutionxparams 
Consider the directed graph created by placing an edge from a node to each
node it would infect if given the opportunity.  $v$ is susceptible at
generation $g$ iff $v$ was initially susceptible, and no ancestor of
$v$ was infected by generation $g-1$.

The probability a randomly chosen ancestor was susceptible at
generation $g-1$ is $S(g-1)/N$.  If $p_i$ is the probability of having
$i$ ancestors, then the probability of being susceptible at generation
$g$ is
\[
\sum_i p_i \left(\frac{S(g-1)}{N}\right)^i
\]
but this is just $\chi(S(g-1)/N)$.
\end{solutionx}
\begin{solutionx}\solutionxparams 
We have $\lim_{g\to\infty} S(g) = \lim_{g\to\infty}(1-\rho) N
\chi(S(g-1)/N)$ or $S(\infty) = (1-\rho) N \chi(S(\infty)/N)$.
Substituting $r(\infty)  = (N-S(\infty)/N)$ yields
\[
r(\infty) =  1- (1-\rho) \chi(1-r(\infty))
\]
\end{solutionx}
\begin{solutionx}\solutionxparams 
\mbox{}
\begin{myenumerate}
\item $\psi(x)$ is simply $x$ and $\ave{K}=1$.  We have
\begin{align*}
S &= N(1-\rho) \theta\\
I & = N\left( 1- (1-\rho)\theta + \frac{\gamma }{\beta} \ln
    \theta \right)\\
R &= - \frac{\gamma N }{\beta} \ln \theta\\
\dot{\theta} &= - \frac{\beta I }{N} \theta
\end{align*}
\item Exponentiating the equation for $R$ yields
\begin{align*}
\theta(\infty) &=
  \exp (-\beta R(\infty)/\gamma N )\\
& = \exp(-\Ro
  r(\infty))
\end{align*}
So we have $\theta(\infty)$ in terms of $r(\infty)$.  Now
\begin{align*}
r(\infty) &= 1- S(\infty)/N \\
&= 1- N(1-\rho)\theta(\infty)/N \\
&=  1- (1-\rho)\theta(\infty)\\
&= 1- (1-\rho) e^{-\Ro r(\infty)}
\end{align*}
\item This generalizes the result of Theorem~\ref{thm:chi_final} for
arbitrary $\rho$.
\end{myenumerate}
\end{solutionx}
\begin{solutionx}\solutionxparams 
\mbox{}
\begin{myenumerate}
\item If $\dot{S}+\dot{R}=0$, then
\[
N(1-\rho)\dot{\theta} - \frac{\gamma N}{\beta} \frac{1}{\theta}
  \dot{\theta} = 0
\]
Factoring out $N \dot{\theta}$ and taking $\Ro = \beta/\gamma$, we are left
\[
(1-\rho) - \frac{1}{\Ro \theta} = 0
\]
So
\[
\theta = \frac{1}{\Ro(1-\rho)}
\]

Then peak prevalence is
\[
N\left( 1- \frac{1}{\Ro} + \frac{1}{\Ro} \ln
  \frac{1}{\Ro(1-\rho)}\right) = N\left( 1- \frac{1}{\Ro} -
  \frac{1}{\Ro} \ln \Ro(1-\rho) \right)
\]
\item At peak incidence $-\dot{S}$ takes a maximum.  That is,
  $-\dot{\theta}$ is a maximum.  So we need $\diff{}{t} I \theta=0$.
  That is,
\begin{align*}
0 &= \diff{}{t} \left( \theta - (1-\rho)\theta^2 + \frac{\theta}{\Ro}
    \ln \theta\right)\\
&= \dot{\theta} - (1-\rho)2\theta\dot{\theta} +
  \frac{\dot{\theta}}{\Ro}\ln \theta + \frac{1}{\Ro} \dot{\theta}
\end{align*}
Factoring out $\dot{\theta}$ yields
\[
0 = 1 - 2(1-\rho)\theta + \frac{\ln \theta}{\Ro}  + \frac{1}{\Ro}
\]
So
\[
\theta = \frac{1 + (\ln \theta + 1)/\Ro}{2(1-\rho)}
\]
This needs to be solved numerically.  Then plugging this result for
$\theta$ in $-\dot{S} = -(1-\rho)\beta
N\left(1-(1-\rho)\theta+\frac{1}{\Ro} \ln \theta \right)\theta$ yields the peak incidence.
\end{myenumerate}
\end{solutionx}
\begin{solutionx}\solutionxparams 
\mbox{}
\begin{myenumerate}
\item $f$ is the PGF for the Poisson distribution
\[
f_u(x) = \exp \left( \beta \kappa_u\frac{\int_0^t I(\tau) \,
  \mathrm{d}\tau}{N\ave{K}}  (x-1)\right)
\]
\item The probability of still be susceptible is the probability of
  having received $0$ transmissions, which in turn is the coefficient
  of $x^0$ in the series expansion of $f_u(x)$.  This is found by
  setting $x=0$.
\item $f_u(0) = exp \left( -\beta \kappa_u\frac{\int_0^t I(\tau) \,
  \mathrm{d}\tau}{N\ave{K}} \right)$
\end{myenumerate}
\end{solutionx}
\begin{solutionx}\solutionxparams 
\mbox{}
\begin{myenumerate}
\item
By direct observation
\[
\dot{\theta} = -\frac{\beta I(t)}{N } e^{-\beta \int_0^t I(\tau)
  \mathrm{d}\tau/N} = -\beta I\theta/N
\]
and dividing by $\theta$ and susbtituting $\dot{R} = \gamma I$ gives
\[
\dot{\theta}/\theta = -\beta \dot{R}/N\gamma
\]

\item The operations yield
\[
\dot{S}/\theta + \beta I S/N\theta = 0
\]

So
\begin{align*}
\diff{}{t}  S/\theta &= \frac{\dot{S}}{\theta} - S
                       \dot{\theta}/\theta^2\\
&= -\beta I S/N\theta - S \beta I \theta/N\theta^2\\
&= 0
\end{align*}
\item Since $\dot{R} =\frac{ N\gamma}{\beta}\dot{\theta}/\theta$
we have $R = R(0) + \frac{N\gamma}{\beta} \ln \theta $
\item Since $\diff{}{t} S/\theta=0$, we have $S= S(0) \theta$.
\item So $I = N - S(0)\theta -  R(0) - \frac{N\gamma}{\beta} \ln \theta$.
\end{myenumerate}
\end{solutionx}
\begin{solutionx}\solutionxparams 
\mbox{}
We write
\[
\dot{S}_\kappa + \beta \kappa \frac{I}{N\ave{K}} S_\kappa = 0
\]
and multiply by $1/\theta^\kappa$.  Then
\[
\diff{}{t} \frac{S_\kappa}{\theta^\kappa} = 0
\]
and
\[
S_\kappa(t) = S_\kappa(0) \theta^\kappa
\]

We assume that $\psi(x) = \sum_\kappa P(\kappa) x^\kappa$. where
$P(\kappa) = N_\kappa/N$.  Starting with a fraction $1-\rho$ randomly
infected yields our expression for $S = \sum_\kappa S_\kappa(t)$.

Since $\dot{R} = \gamma I$ and $\dot{\theta} = -\beta I \theta/N$, we
can substitute to find $\dot{R} = -\gamma N \dot{\theta}/\theta
\beta$.  This can be integrated to find $R$ in terms of $\theta$.

Then simply set $I = N - S - R$ to complete the calculation.
\end{solutionx}
\begin{solutionx}\solutionxparams 
\mbox{}
\begin{myenumerate}
\item \begin{itemize}
\item $\psi_1(x_1,x_2) = e^{\lambda(x_2-1)}$  (independent of $x_1$)
\item $\psi_2(x_1,x_2) = \frac{1-\pi}{1-\pi x_1}$  (independent of
  $x_2$)
\end{itemize}
\item $\vec{\psi}(\vec{x}) = \left(e^{3(x_2-1)},
    \frac{1}{2- x_1}\right)$.  Starting with $\vec{x}=(0,0)$, and
  iterating until convergence we have $\vec{x} = (0.2868, 0.5837)$.
  So the epidemic probability is $0.7132$ starting from a human and
  $0.4163$ starting from a vector.
\end{myenumerate}
\end{solutionx}
\begin{solutionx}\solutionxparams 
\mbox{}
\begin{myenumerate}
\item We have
\begin{align*}
\dot{S}_i &= - \frac{S_i}{N_i}\sum_j \beta_{ij} I_j\\
\dot{S}_i + \left (\frac{\sum_j \beta_{ij} I_j}{N_i}\right) S_i &= 0\\
\diff{}{t} S_i e^{\xi_i}
          &=0\\
S_i = S_i(0) e^{-\xi_i}
\end{align*}
where $\dot{\xi}_i = \sum_j \beta_{ij} I_j/ N_i$.

It is straightforward to add $\dot{R}_i = \gamma_i I_i$ and $I_i = N_i
- S_i - R_i$.
\end{myenumerate}
\end{solutionx}
\begin{solutionx}\solutionxparams 
\mbox{}
\begin{myenumerate}
\item People in group $i$ interact with others at rate $\kappa_i$, and they
  choose their partners at random at each time from the
  entire population with probability proportional to the partner's
  interaction rate.
\item This can be derived directly from an integrating factor or by
  simply substituting in and checking that the ODEs are satisfied.
\item If we move the $S$ and $R$ terms to the right hand side, the
  numerator becomes $\sum_j \kappa_j (I_j +S_j + R_j) = \sum_j \kappa_j
  N_j$.
\item We have $S_j = N_j \theta^\kappa_j$  So
\begin{align*}
\kappa_j S_j &= \kappa_j
  \theta^{\kappa_j} \\
&= \theta \diff{}{\theta} \theta^{\kappa_j}
\end{align*}
Thus summing the terms in the numerator gives $\theta
\psi'(\theta)$.  The denominator can be foundsimilarly.
\item If we substitute $\gamma I_j$ for $\dot{R}_j$ and compare with
  the $\dot{\theta}$ equation the ODE is shown.  Then integrating both
  sides gives $\sum_j \kappa_j R_j/ \sum_j \kappa_j N_j =
  (\gamma/\beta) \ln \theta$.
\item We simply substitute the results of~\textbf{\ref{d}}
  and~\textbf{\ref{e}} into~\textbf{\ref{c}}.  Then substitute this
  into the $\dot{\theta}$ equation from~\textbf{\ref{b}}.
\end{myenumerate}
\end{solutionx}
\begin{solutionx}\solutionxparams 
We first find
\begin{align*}
\left(\diff{}{x}\right)^n f(x) &= \left(\diff{}{x}\right)^n \sum_m r_m
                                 x^m\\
&= \sum_m \left(\diff{}{x}\right)^n r_m x^m\\
&= \sum_m m(m-1)\cdots(m-n+1) r_m x^{m-n}
\end{align*}
\begin{itemize}
\item if $m<n$, one of the terms in the product $m(m-1) \cdots (m-n+1)$
is zero.
\item if $m=n$ then $m(m-1) \cdots(m-n+1)$ becomes $n!$, and $x^{m-n}$
  is simply $1$.
\item if $m>n$, then there is a nonzero factor in front and a factor
  of $x^{m-n}$.
\end{itemize}
When we evaluate this derivative at $x=0$, the terms which are
already zero remain zero, the $m=n$ term remains unchanged, and the
other terms all have $0$ raised to a positive power so they become
zero.

Thus we are left $r_n$.

\end{solutionx}
\begin{solutionx}\solutionxparams 
\mbox{}
\begin{myenumerate}
\item Substituting we have
\begin{align*}
\int_0^1
  \frac{f(Re^{2 \pi i u})}{R^n e^{2 n \pi i u}} \, \mathrm{d}u &= \int_0^1
  \frac{\sum_m r_m (Re^{2 \pi i u})^m}{R^n e^{2 n \pi i u}} \,
                                                                 \mathrm{d}u\\
&= \sum_m  r_m\int_0^1 R^{m-n}e^{2(m-n)\pi i u} \, \mathrm{d}u
\end{align*}
\item For $m=n$, both $R^{m-n}$ and $e^{2(m-n)\pi i u}$ become $1$.
  Thus we have $\int_0^1 1 \mathrm{d}u = 1$.
\item For $m\neq n$, the integral becomes
\begin{align*}
\int_0^1 R^{m-n}e^{2(m-n)\pi i u} \, \mathrm{d}u &=
                                                   R^{m-n}\int_0^1e^{2(m-n)\pi
                                                   i u} \,
                                                   \mathrm{d}u\\
&=  R^{m-n}\int_0^1e^{2(m-n)\pi i u} \, \mathrm{d}u\\
&=  R^{m-n}\frac{1}{2(m-n)\pi i} \left( e^{2(m-n)\pi i 1} -
  e^{2(m-n)\pi i 0}\right)\\
&= R^{m-n} \frac{1}{2(m-n)\pi i} (1-1)\\
&=0
\end{align*}
where in the last step we use the fact that $e^{2N\pi i} = \cos 2N\pi
+ i \sin 2N\pi = 1$ for any integer $N$.
\item So the integral $\int_0^1 \frac{f(Re^{2 \pi i u})}{R^n e^{2 n \pi i u}} \, \mathrm{d}u$
  becomes
\begin{align*}
\int_0^1 \frac{f(Re^{2 \pi i u})}{R^n e^{2 n \pi i u}} \, \mathrm{d}u
&= 0r_0 + 0r_1 + \cdots + 0r_{n-1} + 1r_n + 0r_{n+1} + \cdots\\
&= r_n
\end{align*}

\end{myenumerate}
\end{solutionx}
\begin{solutionx}\solutionxparams 
%The script \texttt{integral\_exercise.py} which is given as
%a supplementary file perfoms these calculations.
\begin{myenumerate}
\item $M=2$:
\begin{align*}
r_0 &\approx 1.543\\
r_1 &\approx 1.175\\
r_2 &\approx 1.543\\
r_3 &\approx 1.175\\
r_4 &\approx 1.543\\
r_5 &\approx 1.175
\end{align*}
\item $M=4$:
\begin{align*}
r_0 &\approx 1.042\\
r_1 &\approx 1.008\\
r_2 &\approx 0.5013\\
r_3 &\approx 0.1669\\
r_4 &\approx 1.042\\
r_5 &\approx 1.008
\end{align*}
\item $M=5$:
\begin{align*}
r_0 &\approx 1.008\\
r_1 &\approx 1.001\\
r_2 &\approx 0.5002\\
r_3 &\approx 0.1667\\
r_4 &\approx 0.04167\\
r_5 &\approx 1.008
\end{align*}
\item $M=10$:
\begin{align*}
r_0 &\approx 1.000\\
r_1 &\approx 1.000\\
r_2 &\approx 0.500\\
r_3 &\approx 0.1667\\
r_4 &\approx 0.04167\\
r_5 &\approx 0.008333
\end{align*}
\item $M=20$:
\begin{align*}
r_0 &\approx 1.000\\
r_1 &\approx 1.000\\
r_2 &\approx 0.5000\\
r_3 &\approx 0.1667\\
r_4 &\approx 0.04167\\
r_5 &\approx 0.008333
\end{align*}
\item Convergence is quite fast, and predicts $r_n$ quite well once $M > n$.
\end{myenumerate}
\end{solutionx}
\begin{solutionx}\solutionxparams 
As in the example, we take $\alpha_g$ to be the probability of failure
within the first $g$ flips, with $\alpha_0=0$ and $\alpha_1=1-p =
f(0)$.

If the first flip does not come up as ``failure'', then the
probability that failure occurs within the following $g-1$ flips is
(by definition) $\alpha_{g-1}$.  So the probability of failure within
the first $g$ flips is the probability of failure in the first flip
plus the probability of success time $\alpha_{g-1}$. That is:
\[
\alpha_{g} = (1-p) + p \alpha_{g-1}  = f(\alpha_{g-1})
\]
\end{solutionx}
\begin{solutionx}\solutionxparams 
\mbox{}
\begin{myenumerate}
\item The probability of dying out after $g$ iterations is the sum
  over all $i$ of the probability that the first roll is an $i$ and
  the process dies out after $g-1$ iterations.  By thinking of each
  die that rolls an $i$ as having $i$ ``offspring'' we can assign each
  individual a collection of descendants.  The process goes extinct
  after $g$ iterations if
  all the dice in the second roll have no offspring after $g-1$ iterations.
\[
\sum_{i=0}^6 \frac{1}{6} \alpha_{g-1}^i = f(\alpha_{g-1}) = f^{[g]}(0)
\]
\item This is equivalent to a disease for which each individual causes
  $0$, $1$, $2$, $3$, $4$, or $5$ new infections with equal
  probability.  So the extinction probability for such a disease is $f^{[g]}(0)$.
\end{myenumerate}
\end{solutionx}
\begin{solutionx}\solutionxparams 
We re-express the negative binomial by interchanging what we count as a
failure and success.  We seek the number of failures that occur before
the $\hat{r}$th success.  We say a success occurs with probability $\hat{p}$ and
failure with probability $\hat{q}=1-\hat{p}$ (which satisfy $\hat{p} =
q$, \ $\hat{q}=p$).

The result for the geometric distribution says that the number of
failures between each success has PGF $\hat{p}/(1-\hat{q}x)$.  We need
the sum of $\hat{r}$ of these.  So by Property~\ref{prop:composition},
we have that the negative binomial has PGF
$[\hat{p}/(1-\hat{q}x)]^{\hat{r}}$.  Replacing $\hat{p}$ by $q$ and
$\hat{q}$ by $p$ completes the result.
\end{solutionx}
\begin{solutionx}\solutionxparams 
\mbox{}
\begin{myenumerate}
\item Because each $i$ in $1, 2, \ldots, 6$ has probability $1/6$, we
  have $f(x) = \sum_{i=1}^6 (1/6) x^i$.
\item
\begin{center}
\begin{tabular}{Sc||Sc|Sc|Sc|Sc|Sc|Sc|}
& $1$ & $2$ & $3$ & $4$ & $5$ & $6$\\
\hline
\hline
$1$ &$2$&$3$&$4$&$5$&$6$&$7$\\
\hline
$2$ &$3$&$4$&$5$&$6$&$7$&$8$\\
\hline
$3$ &$4$&$5$&$6$&$7$&$8$&$9$\\
\hline
$4$ &$5$&$6$&$7$&$8$&$9$&$10$\\
\hline
$5$ &$6$&$7$&$8$&$9$&$10$&$11$\\
\hline
$6$ &$7$&$8$&$9$&$10$&$11$&$12$\\
\hline
\end{tabular}
\hspace{1in}
\begin{tabular}{Sc||Sc|Sc|Sc|Sc|Sc|Sc|}
& $x^1$ & $x^2$ & $x^3$ & $x^4$ & $x^5$ & $x^6$\\
\hline\hline
$x^1$ &$x^2$&$x^3$&$x^4$&$x^5$&$x^6$&$x^7$\\
\hline
$x^2$ &$x^3$&$x^4$&$x^5$&$x^6$&$x^7$&$x^8$\\
\hline
$x^3$ &$x^4$&$x^5$&$x^6$&$x^7$&$x^8$&$x^9$\\
\hline
$x^4$ &$x^5$&$x^6$&$x^7$&$x^8$&$x^9$&$x^{10}$\\
\hline
$x^5$ &$x^6$&$x^7$&$x^8$&$x^9$&$x^{10}$&$x^{11}$\\
\hline
$x^6$ &$x^7$&$x^8$&$x^9$&$x^{10}$&$x^{11}$&$x^{12}$\\
\hline
\end{tabular}.
\end{center}
\item Multiplication of two powers of $x$ results in addition of the exponents.
\item We have
\begin{align*}
x(1+x+x^2)(1+x^3) &=  x(1+x+x^2+x^3+x^4+x^5)\\
&= x+x^2+x^3+x^4+x^5+x^6
\end{align*}
and
\begin{align*}
(1+x)(1-x+x^2) &= 1 -x + x^2 +x-x^2+x^3\\
&= 1+x^3
\end{align*}
\item Since the PGF of the sum of the two dice is equal to the product
  of the PGFs of the two dice, we must have $h_1(x)h_2(x)=[f(x)]^2$.
\item For each die, the probabilities of the sides are $1/6$.  So they
  take the form $\sum_i x^{a_i}/6$ and $\sum_i x^{b_i}/6$.
\item Because each $a_i$ and $b_i$ is positive $\sum_i 0^{a_i}/6$ and
  $\sum_i 0^{b_i}/6$ are both $0$.
\item $\sum_i 1^{a_i}/6 = 1$ and $\sum_i 1^{b_i}/6=1$.
\item Because $h_1(0)=h_2(0)=0$, both of them must have a factor of
  $x$.  Because $h_1(1)=h_2(1)=1$ and the denominators are $6$, the
  numerators when $x=1$ must be $6$.  So there must be a factor of $2$
  and $3$ in the numerator.  This requires that each has a single factor of
  $(1+x+x^2)$ and $(1+x)$.  Because $1-x+x^2$ is $1$ when $x=1$,
  they could have a factor of $(1-x+x^2)^{2-b}$ for $b=0$, $1$, or
  $2$.
\item Taking $b=0$ we have
\begin{align*}
h_1(x) &= x(1+x+x^2)(1+x)/6\\
 &=\frac{x(1+2x+2x^2+x^3)}{6}\\
&= \frac{x+x^2+x^2+x^3+x^3+x^4}{6}\\
\end{align*}
The calculation for $h_2(x)$ is not asked for in the question, but it is
\begin{align*}
h_2(x) &= h_1(x) (1-x+x^2)(1-x+x^2)\\
&= h_1(x)(1 -x+x^2-x+x^2-x^3+x^2-x^3+x^4)\\
&= \frac{x+2x^2+2x^3+x^4}{6}(1-2x+3x^2-2x^3+x^4)\\
&= \frac{1}{6} \big( x -2x^2+3x^3-2x^4+x^5\\
&\qquad\quad +2x^2- 4x^3+6x^4-4x^5+2x^6 \\
&\qquad\qquad\qquad+ 2x^3-4x^4+6x^5-4x^6+2x^7\\
&\qquad\qquad\qquad\qquad\quad + x^4 -2x^5 + 3x^6 - 2x^7 + x^8\big)\\
&=\frac{1}{6}(x + x^3 +x^4+x^5+x^6+x^8)
\end{align*}
\item \begin{tabular}{Sc||Sc|Sc|Sc|Sc|Sc|Sc|}
 &$1$&$2$&$2$&$3$&$3$&$4$\\
\hline\hline
 $1$&$2$&$3$&$3$&$4$&$4$&$5$\\
\hline
 $3$&$4$&$5$&$5$&$6$&$6$&$7$\\
\hline
 $4$&$5$&$6$&$6$&$7$&$7$&$8$\\
\hline
 $5$&$6$&$7$&$7$&$8$&$8$&$9$\\
\hline
 $6$&$7$&$8$&$8$&$9$&$9$&$10$\\
\hline
 $8$&$9$&$10$&$10$&$11$&$11$&$12$\\
\hline
\end{tabular}
The sums all occur with the same frequency as a normal pair.

If we didn't calculate $h_2(x)$ in the previous part, we could have
inferred the values from knowing what the first die was and what
values would be needed to match the normal pair.
\end{myenumerate}
\end{solutionx}
\begin{solutionx}\solutionxparams 
\mbox{}
\begin{myenumerate}
\item By Property~\ref{prop:composition}, the PGF is $f(f(x))$.
\item This is equivalent to the dice-rolling example.  It is
  $f(f(x))$.
\item More generally for generation $g$, we have $f^{[g]}(x)$.
\end{myenumerate}
\end{solutionx}
\begin{solutionx}\solutionxparams 
\mbox{}
\begin{myenumerate}
\item For $z(x)=2(1-x)/3$ with $x_0=0$, the cobweb diagram spirals in
  towards $0.4$,  the solution to $x=z(x)$.  \raisebox{-0.5\height}{\includegraphics[scale=0.3]{cobweb_exercise0.pdf}}
\item For $z(x)=2(1-x)$ with $x_0=0.664$, the cobweb diagram spirals
  away from $2/3$, the solution to  $x=z(x)$.  \raisebox{-0.5\height}{\includegraphics[scale=0.3]{cobweb_exercise1.pdf}}
\item For $z(x)=1/4 + x/2$, the cobweb diagram steps in to $x=1/2$, the solution $x=z(x)$. \\ \raisebox{-0.5\height}{\includegraphics[scale=0.3]{cobweb_exercise2.pdf}}\\
For $z(x)=-1+3x$, the cobweb diagram steps away from $x=1/2$, the solution $x=z(x)$.  \raisebox{-0.5\height}{\includegraphics[scale=0.3]{cobweb_exercise3.pdf}}
\item When the slope is positive, each successive value is on the same
  side of the intercept.  When it is negative the values alternate.
\item If we take $x^*$ to be the solution $x^*=z(x^*)$, then when $|z'(x^*)|>1$ the values diverge from $x^*$, while
  when $|z'(x^*)|<1$ they converge.
\item Sufficiently close to the intersection where $x^*=z(x^*)$,
  we can locally treat $z(x)$ as a
  line.  If $z'(x^*)$ is $1$ at this intersection, this line lies on top
  of $z(x)=x$ and the correction to the line makes a difference.  For all other values
  the nonlinear terms can be neglected.
\end{myenumerate}
\end{solutionx}
\begin{solutionx}\solutionxparams 
\mbox{}
\begin{myenumerate}
\item $f(1) = \sum_i r_i 1^i = \sum_i r_i = 1$ because the $r_i$ form
  a probability distribution and $f(0) = \sum_i r_i 0^i = r_0 >0$.
\item $f''(x) = \sum_i i(i-1) r_i x^{i-2}$.  Because $r_i \geq 0$ and
  $x \geq 0$  this sum is $\geq 0$.  [the inequality is strict if any
  $r_i >0$ for $i \geq 2$].
\item Note first that $f(1)=1$.  If $f'(1)\leq 1$, then for all $x$
  in $0 \leq x < 1$, we have $f'(1) < 1$.  So because the line $y=x$
  has a larger slope, it lies strictly below $f(x)$ for all $x$ in
  $[0,1)$.  [a more rigorous argument can be made using the mean value
  theorem: assume some $x_0$ in $[0,1)$ has $f(x_0)=x_0$.  Then by the
  mean value theorem there is an $\hat{x} \in (x_0, 1)$ where
  $f'(\hat{x})$ is equal to the slope of the line connecting the
  points $(x_0, f(x_0))$ and $(1, f(1))$.  This line is $y=x$, and has
  slope $1$, so $f'(\hat{x})=1$.  No such $\hat{x}$ exists, so the
  assumption that such an $x_0$ exists must be false.]
\item $f'(x_0)>0$ because $f'(x_0) = \sum_i i r_i x^{i-1}$ and unless
  $r_0=1$, this is strictly positive.  If $r_0=1$, then $f(x)=1$ and
  no such $x_0$ exists.  To show $f'(x_0) <1$, note that for $f(x)$ to
  be less than $x$ for $x>x_0$, but equal to $x$ for $x=x_0$, it
  must have smaller slope than that of $y=x$ [a more rigorous proof uses the
  mean value theorem to show that there is an $\hat{x} \in (x_0, x_1)$
  with slope $<1$ and so since $f''(x)>0$, we have $f'(x_0) < f'(\hat{x})<1$.].
\item Again we start with the observation that $f(1)=1$.  Because
  $f'(x) >1$ at $x=1$, there must be a region $(\hat{x}, 1)$ such that if
  $x \in (\hat{x}, 1)$ then $f(x) < x$ as it has greater slope than the
  line $y=x$ [again, a more rigorous proof would use the mean-value
  theorem, and the fact that $f'(x)$ is continuous at $1$].  However,
  for the curve $f(x)$ to reach $f(0)>0$ at $x=0$, it must somewhere
  cross the line [rigorously, we can use the intermediate value
  theorem applied to the function $f(x)-x$ with the point $x=0$ and
  some $x  = x_1 \in (x_0, 1)$].  At the point $x_0$ where $f(x)$ crosses
  $y=x$, our previous result shows that $f'(x_0)< 1$.  So for $x \in
  (0, x_0)$ we have $f'(x)<1$ as well.  Thus $f(x)$ cannot cross $y=x$
  at any other point in $(0,x_0)$ [again, the mean value theorem does
  this more rigorously: if it did cross again, then we could prove
  some $\hat{x} \in (0, x_0)$ where $f'(\hat{x})=1$].
\end{myenumerate}
\end{solutionx}
\begin{solutionx}\solutionxparams 
\mbox{}
\begin{myenumerate}
\item We simply look at the rate $r_i$ is decreasing due to events
  that move the system out of state $i$ plus the rate it increases due
  to events that move the system into state $i$.  The total rate
  moving out is $\sum_m \lambda_m i r_i$.  The total rate in is
  $\sum_m \lambda_m (i-m+1) r_{i-m+1}$.
\item
 \begin{align*}
 \dot{f}(x,t) &= \sum_i \dot{r}_i x^i\\
&= \sum_i \left(- \sum_m \lambda_m i r_i + \sum_m \lambda_m
  (i-m+1) r_{i-m+1}\right) x^i\\
&= - \sum_{i}\sum_m \lambda_m i r_i x^i + \sum_i\sum_m \lambda_m
(i-m+1)r_{i-m+1}x^i\\
&= -\Lambda \sum_i i r_i x^i + \sum_m \lambda_m \sum_i (i-m+1)
r_{i-m+1}x^i\\
&= -\Lambda x \sum_i i r_i x^{i-1} + \sum_m \lambda_m x^{m}\sum_i (i-m+1)
r_{i-m+1} x^{i-m}\\
&= -\Lambda x \pd{}{x} \sum_i r_i x^i + \sum_m \lambda_m x^m \pd{}{x} \sum_i
r_{i-m+1}x^{i-m+1}\\
&= -\Lambda x \pd{}{x} f(x,t) + \sum_m \lambda_m x^m \pd{}{x} f(x,t)\\
&= -\Lambda x \pd{}{x} f(x,t)+ \Lambda h(x) \pd{}{x} f(x,t)\\
&= \Lambda(h(x)-x) \pd{}{x} f(x,t)
\end{align*}

\end{myenumerate}
\end{solutionx}
\begin{solutionx}\solutionxparams 
\mbox{}
\begin{myenumerate}
\item Let $\beta_{m} i(i-1)$ denote the rate at which the system
  goes from a state with $i$ individuals to $i-2+m$ individuals (that
  is, two individuals are replaced by $m$).  Then
\begin{align*}
f(x,t+\Delta t) &= \sum_i r_i(t) \left[ \sum_m (\beta_m i(i-1) \Delta t
  )x^{i+m-2} + \left(1- \sum_m \beta_m i(i-1) \Delta t\right)
  x^i\right]  + \littleo(\Delta t)\\
&= \sum_i r_i x^i + \sum_m \beta_m (\Delta t) (x^m-x^2) \sum_i r_ii(i-1)
x^{i-2} + \littleo(\Delta t)\\
&= f(x,t) + \mathfrak{B}\Delta t [g(x) - x^2] \sum_i r_i i(i-1)
x^{i-2} + \littleo(\Delta t)\\
&= f(x,t) + \mathfrak{B} \Delta t[g(x)-x^2] \pds{}{x} f(x,t) +
\littleo(\Delta t)
\end{align*}
Plugging this into
\[
\pd{}{t} f(x,t) = \lim_{\Delta t \to 0} \frac{f(x,t+\Delta t)-f(x)}{\Delta t}
\]
yields
\[
\pd{}{t} f(x,t) = \mathfrak{B} [g(x)-x^2] \pds{}{x} f(x,t)
\]
\item The proof is almost the same as the previous case:
Let $\beta_{m} i^2$ denote the rate at which the system
  goes from a state with $i$ individuals to $i-2+m$ individuals (that
  is, two individuals are replaced by $m$).  Then
\begin{align*}
f(x,t+\Delta t) &= \sum_i r_i(t) \left[ \sum_m (\beta_m i^2 \Delta t
  )x^{i+m-2} + \left(1- \sum_m \beta_m i^2 \Delta t\right)
  x^i\right]  + \littleo(\Delta t)\\
&= \sum_i r_i x^i + \sum_m \beta_m (\Delta t) (x^m-x^2) \sum_i r_ii^2
x^{i-2} + \littleo(\Delta t)\\
&= f(x,t) + \mathfrak{B}\Delta t [g(x) - x^2] \sum_i r_i i^2
x^{i-2} + \littleo(\Delta t)\\
&= f(x,t) + \mathfrak{B} \Delta t[g(x)-x^2] \frac{1}{x}\pd{}{x} x\pd{}{x} f(x,t) +
\littleo(\Delta t)
\end{align*}
Plugging this into
\[
\pd{}{t} f(x,t) = \lim_{\Delta t \to 0} \frac{f(x,t+\Delta t)-f(x)}{\Delta t}
\]
yields
\[
\pd{}{t} f(x,t) = \mathfrak{B} [g(x)-x^2] \frac{1}{x}\pd{}{x} x \pd{}{x}f(x,t)
\]
\end{myenumerate}
\end{solutionx}
\begin{solutionx}\solutionxparams 
\begin{align*}
\pd{}{t} f(x,y,t) &= \xi (x^{-1}y - 1)x \pd{}{x} f(x,y,t) + \eta (x^{-1}y-1) xy\pd{}{x}\pd{}{y}f(x,y,t)\\
&= \left(\xi (y-x) \pd{}{x} + \eta (y^2-xy) \pd{}{x}\pd{}{y}\right) f(x,y,t)
\end{align*}
\end{solutionx}
\begin{solutionx}\solutionxparams 
\mbox{}

\begin{myenumerate}
\item \begin{align*}
f_{1,0}(x,y,\Delta t) &= \sum_i r_{i,j}(0) x^i \left(1 - \sum_{m,n} i
  \lambda_{m,n} \Delta t + \sum_{m,n}  i \lambda_{m,n} x^{m-1}y^n\right) +
  \littleo(\Delta t)\\
&= x\left( 1 - \sum_{m,n}
  \lambda_{m,n} \Delta t + \sum_{m,n}   \lambda_{m,n} x^{m-1}y^n\right) +
  \littleo(\Delta t)\\
&= x - x(\Delta t) \sum_{m,n} \lambda_{m,n} + \sum_{m,n}\lambda_{m,n} x^m y^n +
\littleo(\Delta t)\\
&= x + (\Delta t) \Lambda [h(x,y) - x] + \littleo(\Delta t)
\end{align*}
Similarly
\[
f_{0,1}(x,y,\Delta t) = y + (\Delta t) \mathfrak{Z} [g(x,y)-y] +
\littleo(\Delta t)
\]
\item We find
\[
f_{1,0}(x,y,\Delta t + t) =
f_{1,0}(f_{1,0}(x,y,t),f_{0,1}(x,y,t), \Delta t)
\]
and
\[
f_{0,1}(x,y,\Delta t + t) = f_{0,1}(f_{1,0}(x,y,t), f_{0,1}(x,y,t),
\Delta t)
\]

\item We now have
\begin{align*}
\pd{}{t} f_{1,0}(x,y,t) &= \lim_{\Delta t \to 0}
\frac{f_{1,0}(x,y,\Delta t + t)-f_{1,0}(x,y,t)}{\Delta t} \\
&= \lim_{\Delta t \to 0}
\frac{f_{1,0}(f_{1,0}(x,y,t),f_{0,1}(x,y,t),
\Delta t) -f_{1,0}(x,y,t)}{\Delta t} \\
&=\lim_{\Delta t \to 0}
\frac{ f_{1,0}(x,y,t) + (\Delta t) \Lambda[h(f_{1,0}(x,y,t),f_{0,1}(x,y,t))
- f_{1,0}(x,y,t)]  + \littleo(\Delta t) -f_{1,0}(x,y,t)}{\Delta t} \\
&= \Lambda [h(f_{1,0}(x,y,t), f_{0,1}(x,y,t)) - f_{1,0}(x,y,t)] + \lim_{\Delta t \to 0}
\frac{\littleo(\Delta t)}{\Delta t}\\
&=\Lambda [h(f_{1,0}(x,y,t), f_{0,1}(x,y,t)) - f_{1,0}(x,y,t)]
\end{align*}
Similarly
\[
\pd{}{t} f_{0,1}(x,y,t) = \mathfrak{Z} [g(f_{1,0}(x,y,t),
f_{0,1}(x,y,t))]
\]
\item To derive Equation~\eqref{eqn:backward_result}, we take infected
  individuals to be type $A$ and recovered individuals to be type
  $B$.  We replace $x$ with $\tilde{y}$, and $y$ with $\tilde{z}$.  We will drop the
  tildes later.

  The events that can happen are that a single infected individual can
  be replaced by $2$ infected individuals (with rate $\beta$ per
  infected individual) or by $1$ recovered individual (with rate
  $\gamma$ per infected individual).  So $\Lambda = (\beta + \gamma)$,
  and $h(\tilde{y}, \tilde{z}) = (\beta \tilde{y}^2 +
  \gamma\tilde{z})/(\beta+\gamma)$.  There are no events that can
  happen to recovered individuals, so $\mathfrak{Z} = 0$ and $g$ could
  be anything.

  So
\begin{align*}
\pd{}{t} f_{1,0}(\tilde{y},\tilde{z}, t) &= (\beta+\gamma)
\left[\frac{\beta f_{1,0}(\tilde{y},\tilde{z},t)^2 + \gamma
    f_{0,1}(\tilde{y},\tilde{z},t)}{\beta+\gamma} -
  f_{1,0}(\tilde{y},\tilde{z},t)\right]\\
\pd{}{t} f_{0,1}(\tilde{y},\tilde{z},t) &= 0
\end{align*}
Since $f_{0,1}(\tilde{y},\tilde{z},t)$ is constant and initially it is
simply $\tilde{z}$, we conclude that it is always $\tilde{z}$.  Thus
we get
\[
\pd{}{t} f_{1,0}(\tilde{y},\tilde{z},t) = (\beta+\gamma)
\left[\frac{\beta f_{1,0}(\tilde{y},\tilde{z},t)^2 + \gamma
\tilde{z}}{\beta+\gamma} -
  f_{1,0}(\tilde{y},\tilde{z},t)\right]
\]
Then replacing $f_{1,0}$ by $\Pi$, \ $\tilde{y}$ by $y$ and
$\tilde{z}$ by $z$ and replacing $\frac{\beta f_{1,0}(\tilde{y},\tilde{z},t)^2 + \gamma
\tilde{z}}{\beta+\gamma}$ by $\hat{\mu}(\Pi(y,z,t),z)$ completes the result.
\end{myenumerate}

\end{solutionx}
\begin{solutionx}\solutionxparams 
The offspring distribution is geometric with $q =
\beta/(\beta+\gamma)$.

The result in Table~\ref{table:final_probs}
predicts $j$ infections with probability
\[
\frac{1}{j} \binom{2j-2}{j-1}
\left(\frac{\gamma}{\beta+\gamma}\right)^j
\left(\frac{\beta}{\beta+\gamma}\right)^{j-1} = \frac{1}{j}
\frac{\gamma^j\beta^{j-1}}{(\beta+\gamma)^{2j-1}} \binom{2j-2}{j-1}
\]
\end{solutionx}

